Reconstructing Ultrametric Trees from Noisy Experiments

The problem of reconstructing evolutionary trees or phylogenies is of great interest in computational biology. A popular model for this problem assumes that we are given the set of leaves (current species) of an unknown binary tree and the results of `experiments' on triples of leaves (a,b,c), which return the pair with the deepest least common ancestor. If the tree is assumed to be an ultrametric (i.e., all root-leaf paths have the same length), the experiment can be equivalently seen to return the closest pair of leaves. In this model, efficient algorithms are known for tree reconstruction. In reality, since the data on which these `experiments' are run is itself generated by the stochastic process of evolution, these experiments are noisy. In all reasonable models of evolution, if the branches leading to the leaves in a triple separate from each other at common ancestors that are very close to each other in the tree, the result of the experiment should be close to uniformly random. Motivated by this, we consider a model where the noise on any triple is just dependent on the three pairwise distances (referred to as distance based noise). Our results are the following: 1. Suppose the length of every edge in the unknown tree is at least $\tilde{O}(\frac{1}{\sqrt n})$ fraction of the length of a root-leaf path. Then, we give an efficient algorithm to reconstruct the topology of the tree for a broad family of distance-based noise models. Further, we show that if the edges are asymptotically shorter, then topology reconstruction is information-theoretically impossible. 2. Further, for a specific distance-based noise model--which we refer to as the homogeneous noise model--we show that the edge weights can also be approximately reconstructed under the same quantitative lower bound on the edge lengths.

==> abstract.tex <==
The problem of reconstructing evolutionary trees or phylogenies is of great interest in computational biology. \ade{A popular model} for this problem assumes that we are given the set of leaves (current species) of an unknown binary tree and the results of `experiments' on triples of leaves $(a,b,c)$, which return the pair with the deepest least common ancestor. If the tree is assumed to be an \textit{ultrametric} (i.e., with all root-leaf paths of the same length), the experiment can be equivalently seen to return the closest pair of leaves. In this model, efficient algorithms are known for reconstructing the tree. In reality since the data on which these `experiments' are run is itself generated by the stochastic process of evolution, these experiments are noisy.  In all reasonable models of evolution, if the branches leading to the three leaves in a triple separate from each other at common ancestors that are very close to each other  in the tree,  the result of the experiment should be close to uniformly random. Paralleling the problem set up in the literature on stochastic block models, we ask whether we can reconstruct the tree with high probability when such noisy results of all $\genfrac(){0pt}{2}{n}{3}$ experiments are given. Under this model, we show that if every edge has length at least $\tilde{O} (\frac{1}{\sqrt n})$ fraction of the length of a root-leaf path, we can in fact reconstruct the topology of the tree with high probability. Furthermore, with a slightly stronger lower bound on the lengths of edges, which is still $\tilde{O} (\frac{1}{\sqrt n})$, we show that we can approximate the weights of all edges of the tree. This is in sharp contrast to the noise-free case, where such a reconstruction of weights is impossible. Finally, we prove that our assumption about the edge lengths is necessary; if the edges are asymptotically shorter,  we show that topology reconstruction is information-theoretically impossible.

 %In contrast, there is simply no information to reconstruct the weights in the noise-free case.

 %Finally we prove that  by showing that if edges can be significantly shorter, topology reconstruction is impossible.

==> alg_outline_old.tex <==


\label{sec:topology}

This section is devoted to the proof of the following result.

\begin{theorem}
\label{theorem:topology}
Let $T$ be a weighted full binary tree tree such that the weights induce an ultrametric on the distances between leaves and that the weight on each edge is at least $\tau \fs$, for some large constant $\tau$. Then, given access to the noisy query model, as described in Section~\ref{sec:model}), on the leaves of this tree, we show that there exists an algorithm $\mathsf{A_{Topology Reconstruction}}$ that, with high probability, exactly reconstructs the topology of this tree.
\end{theorem}

We start by providing a high-level description of the algorithm $\mathsf{A_{Topology Reconstruction}}$. We want to infer an unknown tree $T$ on a given set of leaves $L$. We have the ability to perform
queries on triples $(a,b,c) \in L$. This query returns one of the three possible pairs as answers with probabilities ... \sk{Fill in by repeating the more general model here}.
We use the phrase `resolving the topology' of a subtree $T'$ to mean that we know the rooted tree representation of $T'$ (perhaps without having inferred edge weights).

Our algorithm works by resolving the topologies of small subtrees, and then stitching these together until all of $T$ is resolved.

\begin{enumerate}

\item In a bottom-up manner by combining sibling subtrees, we can build a ``base'' tree $T_B$ containing between $\sqrt{n}$ and $2 \sqrt{n}$ leaves that is a subtree of $T$ with high probability. (This is as large a tree as we can build to be confident that we have a subtree of $T$.)

\item We use the same idea to build a "pivot" tree $T_P$  on about the same number of  leaves outside of $L(T_B)$. With high probability, $T_P$ will also be a subtree of the induced tree on $L - L(T_B)$.

\item Using the fact that $|L(T_B) | * |L (T_P)| = \Omega (n)$,  we can partition the leaves in $L(T) - L(T_B)$ into 3 parts (some possibly empty) --- leaves in buckets to the left of  $T_P$ (i.e., buckets with smaller indices than the buckets that the leaves of $T_P$ come from), leaves in the same bucket as $T_P$, and leaves in buckets to the right of $T_P$ (i.e., buckets with smaller indices than the buckets that the leaves of $T_P$ come from).

\item  We show that if a subtree excludes $\Omega (n)$ leaves then we can infer its entire topology with high probability. Likewise, if it contains $\Omega (n)$ leaves, we can infer the topology of the complement of the subtree with high probability. Using these two facts, we fully resolve the topology of all but one of the 3 parts in the previous step and recurse on the unresolved part. When this part has fewer than \sk{Check this bound once the algorithm is completely final.} $\frac{11n}{12}$ leaves, we can infer its topology directly from the leaves outside this part, and the recursion bottoms out.

\end{enumerate}


\hide{
Our approach for reconstructing  $T$ is to find this order with respect to a subtree $T_B$ and then resolve all three-way queries within each partition $S_1, \cdots S_k$, as well as within $T_B$.  %$T_B$ is referred to as the base for the reconstruction.	

Along the way we will have coarser partitions with respect to  $T_B$ that we will iteratively refine. A specific type of coarse partition arises in our algorithm, and we define it below.

\begin{definition}
\label{definition:incomplete}
A reconstruction with base tree $T_B$ is complete except with respect to a contiguous interval $I$ if the following conditions hold:

We know a partial order with respect to $T_1$ where we have a partition $S_{-I}, I, S_{+I}$ of $L(T) - L(T_1)$ such that for all $a \in S_{-I}, c \in S_{+I}, b \in I, x \in T_1$, we know that $d(x,a) < d(x,b) < d(x,c)$. Note that this implicitly shows that $I$ is of the form $S_{i} \cup S_{i+1}\cup \cdots \cup S_{i+j}$ for some contiguous subsequence in the strict weak order with respect to $T_1$. Further, we have refined the leaves in $S_{-I}$ and $S_{+I}$ into buckets, and additionally reconstructed the topologies of all triples within each bucket. This particular type of partial order is shown in Figure~\ref{fig:unknown_contiguous}.
\sk{Might be nice to show that $I$ is somewhat unresolved... the picture shows even the buckets within $I$ as separated.}
\end{definition}

\begin{figure}
    \centering
    \includegraphics[width=8cm]{new_images/unknown contiguous.png}
    \caption{Partial Order with Unknown Contiguous Interval}
    \label{fig:unknown_contiguous}
\end{figure}
}

\hide{    

We first list the main steps of the reconstruction algorithm, and then elaborate on the main ideas behind each of these steps.

\begin{enumerate}

\item Identify a base subtree $T_1$ such that $\sqrt{n} \le |L(T_1)| < 2 \sqrt {n}$. Reconstruct the structure of $T_1$.

\item Repeat the following steps

    \begin{enumerate}
    \item Find the leaves $L(T')$ of a subtree $T'$ of the tree induced by $L(T) - L(T_1)$ such that $\sqrt{n} \le |L(T')| < 2 \sqrt{n}$ While $T'$ might not be a subtree (in our sense) of the overall tree $T$, its leaves form either a contiguous interval of buckets starting with $S_1$ or is a subtree  of the tree induced by the leaves in a single bucket. 
    
    \item Using $L(T_1)$ and $L(T')$, partition $L - L(T_1)$ with respect to $T_1$.  In this partition, either $L(T')$ is the union of a contiguous set of buckets starting from $S_1$ or $L(T')$ is a subset of one bucket.  In the first case all of $L(T) - L(T_1) - L(T')$ lies in higher indexed buckets than $T'$. In the second case, these leaves can lie in one of 3 groups --- those in buckets with lower indices than that of $L(T')$, those in the same bucket as $L(T')$ and those in buckets with higher indices. At most one of the groups has size  $\geq n/2$. Completely resolve all groups with size $< n/2$ and recurse on the large group.
    \end{enumerate}
    
    Until the entire tree is resolved.

    
\end{enumerate}
    


 The main ideas used in the above algorithm are: 1) A large enough subtree can be used to completely resolve the topology of the rest of the tree. In a similar vein, if a subtree \textit{excludes} a sufficient number of leaves, this set of excluded leaves can be used to figure out the topology of the subtree.
 
We first build a small ($\Theta( \sqrt{n})$-sized subtree) $T_1$ as our base by a process of continually identifying and uniting sibling subtrees. This tree serves as our base and the entire remaining set of leaves is the unknown contiguous interval. (The reason we have to stop this process at $\Theta( \sqrt{n})$ is because creating larger trees corrupts the signal necessary for identifying siblings.)  Then, by repeating the process on $L - L(T_1)$,  we find a small subtree $T'$ (of size $\Theta (\sqrt{n})$) of the induced tree formed by the leaves in the unknown contiguous interval. This subtree in the induced tree either corresponds to a contiguous interval within our original strict weak order or to a subset of leaves within one of the buckets in our original strict weak order. %In the  latter case, since the leaves within each bucket form the leaves of a subtree of $T$, the induced subtree $T'$ is in fact also a subtree of $T$. In certain such cases, our algorithm pivots to using the subtree $T'$ as the base subtree for reconstruction. \esh{Have added a line about pivot steps, should we go into greater detail about these cases?} 
We will then use triples involving one leaf from $T_1$ and another from $T'$ (there are $\Omega (n)$ such triples for each $x$ outside of $T_1$ and $T'$) to decide whether $x$ is in a bucket to the left of $T'$ (with respect to the strict weak order  based on $T_1$), in the same bucket as $L(T')$ (in case $T'$ comes from a single bucket), or in a bucket to the right of $T'$. Thus we partition all leaves in $L - L(T_1) - L(T')$ into 1 or 3 classes. All but one of these classes must be of size at most $n/2$, and hence have at least $n/2$ leaves outside the class. Thus we  can completely resolve the topology of all but one of the classes, reducing the size of the unknown contiguous interval. Once the number of leaves in this interval is reasonably small, i.e., less than $\frac{n}{3}$, \sk{replace reasonably small by a precise quantity ... $11n/12$?} \esh{Currently $n/3$, but will fix this after finalizing the algorithm} \esh{Have fixed it to be $n/3$}, we can fully resolve its topology as well, thereby recovering the topology of the entire tree $T$.

Our two primary subroutines have tensions on opposite ends - our small trees building technique is limited to trees of maximum size $O(\sqrt{n})$ while the partitioning algorithm only works when $T_1$ and $T'$ both have $\Omega(\sqrt{n})$. Our overall algorithm exploits this balance to alternately use these subroutines to build up the tree.
}


We prove a simple lemma about sums of independent random variables that will be a useful analytical tool in multiple proofs.


\begin{lemma}
\label{lemma:enough_independent_sum}
Let $L \ge \frac{n}{16}$, let $X_1, X_2, \cdots X_L$ and $Y_1, Y_2,\cdots Y_L$ be two sets of independent $0-1$ random variables such that for all $i \in [L]$, $\E[X_i] \le \E[Y_i] - c \sqrt{\frac{\log n}{n}}$, for a sufficiently large constant $c$. Let $X = \sum_{i=1}^l X_i$ and let $Y = \sum_{i=1}^l Y_i$ Then, with high probability, i.e. at least $1- \frac{1}{n^6}$, we have $Y >X + 24 \sqrt{n \log n}$. 

 Alternatively, if $X_i$ and $Y_i$ are identical random variables for each $i$, with high probability, we have $|X - Y| < 12 \sqrt{n \log n}$.
\end{lemma}


We will now elaborate on the algorithm. 


First, we prove a lemma that establish the claims made in Step 4 above.

\hide{
First we show that given the set of leaves of a large enough subtree $T'$, we can reconstruct the topology of the quotient tree $T/\,T'$. (Recall that this quotient is arrived at by collapsing $T'$ to a single leaf and taking the induced topology on the resulting set of leaves.)
  Next we show that if a subtree excludes a sufficiently large number of leaves, its topology can be reconstructed.
}

\sk{Something is messing up our Lemma and Proof environments... Latex can produce better formatting than this.}

\begin{lemma}
\label{lemma:large_enough}
Let $T$ be a tree with $n$ leaves and $T'$ a subtree.
\begin{enumerate}
\item If $T'$ contains at least $\frac{n}{12}$ leaves, 
given the set $L(T')$, there exists an algorithm that, with high probability, resolves the topology of the quotient $T\,/\,T'$. (Recall that this quotient is arrived at by collapsing $T'$ to a single leaf and taking the induced topology on the resulting set of leaves.)
\hide{a query function $C' : L^3 \rightarrow L^2$ such that for any triple $(a,b,c)$ where at least one of $a, b,$ or $c$
is in $T - T'$, $C'(a,b,c) = C(a,b,c)$. }

\item If $T'$ has at most $\frac{11n}{12}$ leaves, given the set $L(T')$, there exists an algorithm $\mathsf{A_{completion}} $ that, with high probability, resolves  the induced topology on this set with high probability. 
\end{enumerate}

\hide{
a query function $C' : L^3 \rightarrow L^2$ such that $\forall a,b,c \in L(T')$, we have $C'(a,b,c) = C(a,b,c)$.
}


\end{lemma}


\hide{If we know all leaves present in a ``large enough'' subtree $T'$ with $|T'| \ge \frac{n}{12}$, then we can reconstruct the rest of the tree as well as its connections to $T'$, i.e.,  
given the set $L(T')$, we can, whp, recover a query function $Q' : L^3 \rightarrow L^2$ such that for any triple $(a,b,c)$ where at least one of $a, b,$ or $c$
is in $T - T'$, $Q'(a,b,c) = Q(a,b,c)$
}
\hide{
\begin{enumerate}
    \item $\forall a,b,c \in T-T'$, we have $Q'(a,b,c) = Q(a,b,c)$.
    \item $\forall a,b \in T-T', \forall c \in T'$, we have $Q'(a,b,c) = Q(a,b,c)$.
\end{enumerate}
}


\begin{proof}
\input{proofs/goldilocks}
\end{proof}

\hide{
\begin{lemma}
\label{lemma:not_too_large}
If we know all leaves present in a ``not too large '' subtree $T'$ with $|T'| \le \frac{11n}{12}$, then we can reconstruct the structure of the tree $T'$, i.e.,  given the set $L(T')$, we can, whp, recover a query function $C' : L^3 \rightarrow L^2$ such that $\forall a,b,c \in T'$, we have $Q'(a,b,c) = Q(a,b,c)$.
\end{lemma}
}


We now fill in the details of Step 1 in our algorithm outline above, describing and analyzing an algorithm that constructs an approximately $\sqrt{n}$ sized subtree within the induced tree of a  large enough set of leaves.

\begin{lemma}
\label{lemma:build_small_trees}
Given a subset $S \subseteq L$ of leaves with $|S| \ge \frac{n}{12}$,  denoting the (unknown) induced topology on $S$ by $T_S$, whp we can find a subtree $T'$ of  $T_S$ such that $|L(T')| \in [\sqrt{n}, 2 \sqrt{n}]$.
\end{lemma}

\sk{Note that I have changed notation in the statement of this lemma and simplified the statement as well... I didn't like $L'$ for the original set of leaves, since $L'$ seems to go with $T'$. ... so I chose $S$... please fix the notation in the proof consistently.  I changed $T^*$ to $T_S$. Also, I believe that the statement I have now is all you need to imply everything in the more complex statement you had earlier.}

\begin{proof}
\input{proofs/build_trees_updated}
\end{proof}



We show how to partition the leaves within a contiguous interval of buckets onto either side of a $\sqrt{n}$ sized subtree in the induced topology on the leaves within this interval.





\begin{lemma}
\label{lemma:partial_order_refinement}
Let $T_B$ be a subtree of $T$ with $|T_B| \ge \sqrt{n}$ and let $I$ be a contiguous interval in the partition of buckets with respect to $T_B$. Let $T_P$ be a subtree of the tree induced on $L(I)$ with between $\sqrt{n}$ and $2\sqrt{n}$ leaves. Then we can find a partition of $L(I) - L(T_P)$ into 3 sets $P_1, P_2,$ and $P_3$ such that $P_1$ consists of all leaves in lower indexed buckets than the leaves of $T_P$, $P_2$ consists of leaves in the same bucket as $T_P$, and $P_3$ consists of leaves in higher numbered buckets. In the case that $L(T_P)$ comprises leaves from more than one bucket $P_1$ and $P_2$ are empty.
\hide{
\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{new_images/refinement_partition.png}
    \caption{Partition from Lemma~\ref{lemma:partial_order_refinement}}
    \label{fig:refinement partition}
\end{figure}
}
\end{lemma}
\esh{Should we add an (updated) figure for this lemma?}

\begin{proof}
\input{proofs/partition_refinement}
\end{proof}


We now have all the details in place for a full description of the algorithm. The algorithm creates a base tree $T_B$ at the beginning.
We use the same technique to build a subtree $T_P$  of $L(T) - L(T_B)$, also  with $\Theta (\sqrt{n})$ leaves.



For any two leaves $x, y$  not in $L(T_B) \cup L(T_P)$, we will say that $x \preceq_{T_B} y$ iff  $x$'s bucket has index less than or equal to $y$'s.
$x$ and $y$ are in the same bucket iff $x \preceq_{T_B} y$ and $y \preceq_{T_B} x$.  (When the base tree is clear from the context, we will drop the subscript on
the relation symbol.) Using $T_B$ and $T_P$ and the technique in Lemma~\ref{lemma:partial_order_refinement}, we determine the $\preceq$ relationship for all pairs
$x,y \in L - (L(T_B) \cup L(T_P))$. Based on this, we partition these leaves into $P_1, P_2,$ and $P_3$ as described in Lemma~\ref{lemma:partial_order_refinement}.

Since $T_P$ is a subtree of the tree induced on $L - L(T_B)$, there are two possibilities for what $T_P$ looks like with regard to the partition into buckets based on $T_B$.
Either $T_P$ is entirely contained within one of these buckets, or it is the union of an initial interval of buckets.  In the latter case, $P_1$ and $P_2$ are empty.

If the number of leaves in any of the 3 parts is less than $\frac{11n}{12}$ we will say that that part is small. 

\begin{claim} We can resolve the topology of a small part completely with high probability.  
\end{claim}

\begin{proof} \label{claim:finish_the_job}
If $P_1$ is small, noting that $T_B \cup P_1$ form a subtree and appealing to Lemma~\ref{lemma:large_enough} we can infer the topology of $P_1$. If $P_2$ is small, there are two cases: f $P_1$ is large, we can again appeal to Lemma~\ref{lemma:large_enough}, noting that $P_2$ lies outside of a large subtree. Else, $P_3$ must be large, and we once again appeal to Lemma~\ref{lemma:large_enough}, but this time use the fact that $P_2$ is part of a small subtree. Finally, when $P_3$ is small, it is very easy to see how the same Lemma implies that the topology of $P_3$ can be resolved.
\end{proof}

Since there can be at most one small part in the partition, at most one part will be unresolved at the end of this process. Let us call this part $R$. 
In the case the $T_P$ did not lie entirely within one bucket,
$R$ will be $P_3$ (the only non-empty part). 

We now explain how we recursively resolve the topology of this contiguous interval.
If the pivot tree $T_P$ in the current step lies within $R$ (we must be in the case where $T_P$ lies entirely in one bucket, and the unresolved part is this bucket), then we recurse on $R \, / T_P$,  the quotient of $R$ with respect to $T_P$. Since $T_P$ has at most $2 \sqrt{n}$ leaves, the number of nodes in the quotient will still be large.
Also, note 
This recursive call finds a new base tree, a partition with respect to this tree, and so on. If, on the other hand, $T_P$ lies outside of the unresolved part, we recurse on the unresolved part, keeping the same base tree and finding a pivot tree within this part. We will maintain the invariant that $R$ is a contiguous interval of buckets with respect to the current base tree.  If $|R|$  is less than $11n/12$, we can reconstruct it using Claim~\ref{claim:finish_the_job}.

In the case that we change the base, $R$ is an entire bucket, and hence a subtree of the overall tree. Again if $R$ becomes small enough, we can reconstruct it directly by appealing to Lemma~\ref{lemma:not_too_large}.

Thus, we will be able to complete the reconstruction of the whole tree. One final subtle point that the reader may wonder about: Could we lose enough nodes from
the quotient-finding operations that $R$ becomes small while the number of nodes outside of $R$ is also small? A careful accounting shows that this does not happen: Each time we compute a quotient and remove at most $2 \sqrt{n}$ leaves, we have also created a new base tree with at least $\sqrt{n}$ leaves, which lies outide and to the left of $R$. Thus if $R$ becomes small due to the quotient operation, the number of leaves on the left side must be large enough to allow reconstruction of $R$.








\hide{

{\bf Case 1:} $|L(I)| \ge \frac{n}{12}$

First, consider the subcase where $L(I)$ is known to consist of all leaves in a subtree (for instance, this is true right at the beginning and we are aware of this fact). If $|L(I)| \le \frac{11 n}{12}$, we can use Lemma~\ref{lemma:large_enough} to reconstruct the entire tree. Otherwise, we only use Lemma~\ref{lemma:large_enough} to fully reconstruct the tree aside from $I$. Then, we use Lemma~\ref{lemma:build_small_trees} to construct a subtree $T_2$ in the induced tree of the leaves in $I$. Since the leaves in $I$ form a subtree of $T$, $T_2$ is also a subtree of $T$. Now, we do a ``pivot'' step and change the base to $T_2$ by setting $T_1 \leftarrow T_2$. The unknown contiguous interval $I$ is updated to be the the leaves in $L(I) - L(T_2)$.

If $I$ is not known to be a subtree, then we can assume without loss of generality that $ \sqrt{n} \le |T_1| \le 2\sqrt{n}$. This assumption is justified since when we start with $I$ being a subtree, we always pivot to a base of size $\sqrt{n}$ and retain this base, and we only pivot to a different base when we note that $I$ is in fact a subtree. We then use Lemma~\ref{lemma:build_small_trees} to find a set of leaves $T_2$ as stipulated within the induced tree of $I$, and then use Lemma~\ref{lemma:partial_order_refinement} to construct a partition $P_1, P_2, P_3$ of $L(I)-L(T_2)$ based on $T_1$ and $T_2$. $P_1, P_2 \cup T_2$ and $P_3$ are all contiguous intervals with respect to the order defined by $T_1$.  At least one of $P_1, P_2, P_3$ has size at least $\frac{n}{12}$ (since $|T_1|, |T_2| \le 2\sqrt{n}$ and $|I| \ge \frac{n}{3}$). If more than one has size at least $\frac{n}{12}$, then we can do a case wise analysis to show that we can use Lemma~\ref{lemma:large_enough}  to reconstruct the entire tree (not expanded upon here for sake of brevity). 
Using the single large contiguous interval, we can completely resolve the other two unknown contiguous intervals. This can be seen be a case-wise analysis and the use of the suitable part of Lemma~\ref{lemma:large_enough}.  If $|P_1| \ge \frac{n}{12}$, then we can use the subtree whose leaves are the set $L(T_1) \cup L(S_{-I}) \cup P_1$ and the first part of Lemma~\ref{lemma:large_enough} to fully resolve the partitions $P_2$ and $P_3$ (i.e., both their internal topology and the way in which they are connected to the rest of the tree). If $|P_2| \ge \frac{n}{12}$, then since $P_2 \cup L(T_2)$ form the set of leaves of a large subtree, we can use the first part of Lemma~\ref{lemma:large_enough} to fully resolve $P_1$ and $P_2$. Finally, if $|P_3| \ge \frac{n}{12}$, then we know that $T_1 \cup L(S_{-I}) \cup  P_1 \cup L(T_2) \cup P_2$ form the leaves of a subtree that is ``not too large'', thus we can use this subtree and the second part of Lemma~\ref{lemma:large_enough} to fully resolve $P_1$ and $P_2$.
%\esh{Should I expand the casewise analysis?}

We then shrink the unknown interval $I$ by setting it to be the large set $P_1, P_2$ or $P_3$. Additionally, if $P_2$ is the large set, we know that it must be a subtree of $T$, and we record this information to use for a pivot step, at the end of which $T_2$ becomes the new base.


{\bf Case 2 :} $|L(I)| < \frac{n}{3}$

Recall that the total order with respect to $T_1$ is $(S_{-I},I,S_{+I}$). Note that $S_{-I}$ and $S_{+I}$ are already fully resolved. Also, either $|L(T_1) \cup L(S_{-I})| \ge \frac{n}{3}$ or $|L(S_{+I})| \ge \frac{n}{3}$. Consider the former case. Since the leaves in $L(T_1) \cup L(S_{-I})$ form a subtree of $T$, we can use Lemma~\ref{lemma:large_enough} to resolve $I$. Similarly, in the latter case, we know that the leaves in $L(T_1) \cup L(S_{-I}) \cup L(I)$ form a subtree of $T$ and that $|L(T_1) \cup L(S_{-I}) \cup L(I)| \le \frac{2n}{3} < \frac{11n}{12}$. Thus, we can use the second part of Lemma~\ref{lemma:large_enough} to resolve the structure of this tree, and hence $I$.
}

==> comments.tex <==

\begin{comment}
We follow the same template as the algorithm in Section~\ref{section:perfect_trees}, in which we proceed in rounds (indexed from $0$) such that we find the $t$-th cousins of every vertex in round $t$. To do so, we recycle the tests $O^t_a$ from Section~\ref{section:perfect_trees}. However, there is a fundamental difference in the way we approach the case of full binary trees - we can no longer guarantee that we will exactly find $C_t(a)$ in the $t$-th round. What we will instead try to argue is that even if the algorithm makes some errors in the $t$-th round, the errors will be corrected in some future round. Let $C'_i(a)$ represent the set of $i$-th cousins maintained by the algorithm, and let $F'_i(a)$ represent all $j$-th cousins of $a$ with $j \le i$, as maintained by the algorithm. To aid with analysis, let $C^t_i(a)$ represent the $i$-th cousins of $a$, as updated by our algorithm after $t$ rounds. Similarly, let $F^t_i(a)$ represent the set of all $j$-th cousins of $a$ for $j\le i$ as updated by the algorithm after $t$ rounds. Before describing the algorithm, we list the invariants maintained by the algorithm after each round.

\begin{enumerate}
    \item 
    \begin{enumerate}[(a)]
        \item For all leaves $a$, let $MAX_i(a)$ represent the largest index $j \le i$ such that $a$ has a $j$-th cousin. Then, after any round $t$, for all $j \le MAX_t(a)$, $C^t_j(a) = C_j(a)$. Further, for all $MAX_t(a) < j \le t$ and all $i \le MAX_t(a)$, $C^t_j(a) \cap C_i(a) = \phi$ (this is trivially true, since, by definition of $MAX_i(a)$, $C_j(a) = \phi$). 
        \item Implicitly, we have $F_j(a) \subseteq F^t_j(a)$ for all $j \le t$.
        \item $C^t_j(a) = \phi$ for all $j > t$.
        \item If $a,b$ are connected as $i$-th cousins by the algorithms (and remain so as of the end of the $t$-th round), then $F^t_j(a) = F^t_j(b)$ for all $i \le j\le t$. Intuitively, this means that the algorithm constructs a consistent local picture of the graph upto the level of $t$-th cousins for all vertices.
        \item $C'$ remains a symmetric relation, i.e., $b \in C^t_i(a)$ implies that $a \in C^t_i(b)$.
    \end{enumerate}
    \item For all leaves $a$, after $t$ rounds,
    $|F^t_t(a) - F_t(a)| \le \tau \sqrt{n}$, i.e., the number of wrongly paired leaves is never too large. This property is relevant in showing that the tests $O^t_a$ still work as desired despite only having access to $F^{t-1}_{t-1}(a)$ rather than $F_{t-1}(a)$ as was the case in Section~\ref{section:perfect_trees}.
\end{enumerate}

\subsection{The Algorithm}

The algorithm is run for $n+1$ rounds, indexed from $0$ to $n$. We describe the working of the $t$-th round of the algorithm, for all values of $t$ from $0$ to $n$. While we will refer to the tests $O^t_a$, these test will use $F^{t-1}_{t-1}(a)$ rather than $F_{t-1}(a)$ as in the previous section. For convenience, we will set $F_{-1}(a) = F^{-1}_{-1}(a) = C_{i-1}(a) = C^{-1}_{-1}(a) =  a$. Additionally, we will assume that $F^t_i(a)$ and $F_i(a)$ always contains $a$. 

{	
\begin{algorithm}[ht]
	{
		\label{algorithm:full_trees_cousins}
			\caption{Algorithm for Updating $t$-th cousins of all Leaves}
		\begin{algorithmic}[1]
		%\STATE x=5
		\STATE Color all vertices $a$ with $|F'_{t-1}(a)| \ge \frac{2n}{9}$ red, color the remaining vertices blue.
		\STATE For all leaves $a$, construct directed graph $G^t_a$ on the vertex set $L(T) - F'_{t-1}(a)$ in the following manner - evaluate $O^t_a(b,c)$ for all pairs $b,c \in L(T) - F'_{t-1}$. Draw an edge from b to c if $O^t_a(b,c)$ returns $c$.
		%\STATE \COMMENT{Phase 1 of the Algorithm:}
		\STATE Construct directed graph $G^t$  as follows, draw an edge $(a,b)$ if $b$ is a sink in $G^t_a$.
		\FOR{all ordered pairs $ a,b \in L(T)$ such that both edges $(a,b)$ and $(b,a)$ are present in $G^t$}
		\STATE Add $a$ to $C'_t(b)$, $b$ to $C'_t(a)$. 
		\FOR{all $c \in F'_{i-1}(a)$} %\esh{Continue here!!!}
		\IF{$(c,b)$ and $(b,c)$ are edges in $G^t$ and $O^t_a(b,c)$ does not return $c$}
		\STATE Add $c$ to $C'_t(b)$, $b$ to $C'_t(c)$.
		\ELSE
		\STATE Disconnect $a$ and $c$, also disconnect $b$ and $c$ if $c \in F'_t(b)$.
		\ENDIF
		\ENDFOR
		\ENDFOR
		\STATE Prune the $t$-th level connections
		\end{algorithmic}
    }
	\end{algorithm}
}		

The disconnect sub-procedure is defined as follows - for two vertices $(a,b)$, when the procedure is called in the $t$-th round - the procedure essentially removes any previous cousin relationships made between two vertices $a$ and $b$ i.e., if there is any index $j$ such that $a \in C'_j(b)$ (and, implicitly, $b \in C'_j(a)$), these entries are removed.

For sake of explanation, we will refer to the pruning step as the second phase of the algorithm, and everything preceding it as the first phase.

\subsection{The Pruning Step}
Observe that at the start of the pruning step, the $t$-th cousin connections are effectively made between $F'_{t-1}(a)$ and $F'_{t-1}(b)$ for every pair $(a,b)$ that are connected in this step. This is a consequence of the steps taken when connecting any two vertices $a$ and $b$. In the current state, the algorithm can potentially connect a $t-1$ family to more than one $t-1$ family. However, we know that this is not a correct, since we work with a binary tree. Thus, we need to prune such connections and ensure that a $t-1$ family is connected to at most one other $t-1$ family. Each $t-1$ family, associated with a contained leaf vertex $a$ is assigned a score $s(a)$, which counts the number of $t-1$ families it is connected to in this round. If $F'_{t-1}(a)$ has score $s(a)>1$, then all connections except one are discarded - the choice is made by picking the family $F'_{t-1}(b)$ with the smallest possible score $s(b)$, with blue families preferred over red families, in case of ties. If no blue families are present in the tied set, all new connections are discarded. Additionally, connections are retained only if there is two sided agreement ($F'_{t-1}(a)$ chooses $F'_{t-1}(b)$ and $F'_{t-1}(b)$ chooses $F'_{t-1}(a)$). Finally, a connection to family $F''_{t-1}(a)$ is retained only if our rules produce a single choice of family to connect to, otherwise the family is not connected in this round. %We will show in the proof of correctness that this rule selects at most one family (without any further ties to be broken arbitrarily).
\subsection{Proof of Correctness}

First, we show that the invariants suffice to show that the entire tree has been correctly reconstructed when the algorithm terminates, i.e., $C^n_i(a) = C_i(a)$ for all leaves $a$ and all indices $i \in \{0,1,\cdots\}$. Let $U$ be the maximum unweighted height of any vertex in the tree, that is, the unweighted height of the root of the tree.  Note that every leaf has a $U-1$-th cousin, with the root being the least common ancestor. Thus, for all leaves $a$, we have $MAX_{U-1}(a) = U-1$. After the $U-1$-th round, by Invariant 1, we know that for all leaves $a$, $C^{U-1}_i(a) = C_i(a)$ for all indices $i \le U-1$.
Since the root is the highest (in the unweighted height sense) vertex in the graph, no leaf has a $j$-th cousin with $j \ge U$, i.e., $C_i(a) = \phi$ for $i \ge U$. By Invariant 1, we have $C^{U-1}_i(a) = C_i(a) = \phi$ for all $i\ge U$. Consider the execution of the $t$-th round for any $t \ge U$. Our algorithm looks for $t$-th cousins for leaf $a$ in the set $L(T) - F'_{t-1}(a)$. However, we can see by induction that $F'_{t-1}(a) = L(T)$ (starting at the base case of $t=U$ and working onwards). Each graph $G^t_a$ is an empty graph with no vertices, and consequently, no sinks. Thus, no new connections are made and no old connections are disconnected. At the end of the algorithm, we will thus have $C^n_i(a) = C_i(a)$ for all indices $i$ and leaves $a$.


\begin{lemma}
\label{lemma:wrong_leaves}
For all leaves $a$, after $t$ rounds,
    $|F^t_t(a) - F_t(a)| \le \tau \sqrt{n}$, i.e., the number of wrongly paired leaves is never too large.
\end{lemma}

\esh{For now, will assume that the second invariant is true, and add a proof once I have one}

%\begin{corollary}
%\label{corollary:no_change_in_testing}
%$O^t_a(b,c)$ gives the same result when 
%\end{corollary}

We will employ an induction argument to argue the preservation of the first invariant. 

Consider the base case, which is $t=0$. Note that Claim~\ref{claim:local_sibling_ft} is still true, since $F^{-1}_{-1}(a) = F_{-1}(a) = \{a\}$. Thus, at the end of round 1, every agent that has a sibling will be correctly matched to its sibling. However, it is possible that two agents that have a common sibling are matched to each other as siblings.

\begin{comment}


Now, to the induction case - consider the execution of the algorithm in the $t$-th round. 
First, consider the case of leaf $a$ such that $MAX_t(a) =t$, i.e., $a$ has at least one $t$-th cousin. First, we show that if $(a,b)$ are $t$-th cousins, the algorithm actually considers them as a potential pair to connect,i.e., we will argue that $a \notin F^{t-1}_{t-1}(b)$ and $b \notin F^{t-1}_{t-1}(a)$. Note that it is possible that $a$ and $b$ were wrongly connected in the $t'$-th round, where $t'<t$. In that event, we have to show that they are disconnected within the end of the $t-1$-th round. Using Lemma~\ref{lemma:cousin_constraints} , we know that at least one of these vertices, WLOG, $a$, has a $t-1$-th cousin. Using the induction hypothesis, we get that $C^{t-1}_i(a) = C_i(a)$ for all $i \le t-1$. Thus, $b \notin F^{t-1}_{t-1}(a)$. Using the symmetry condition in the induction hypothesis, we get $a \notin F^{t-1}_{t-1}(b)$. This concludes the proof that $a$ is a vertex in $G^t_a$ and $b$ is a vertex in $G^t_a$. Now, we have to argue that they are sinks in the respective graphs, and that leaves that are not first cousins lose out to them in the $O^t$ test.

\begin{lemma}
\label{lemma:correct_cousins}
Given that $a$ and $b$ are $t$-th cousins, we argue that $O^t_a(b,c)$ returns $b$ for all $c \in L(T) - F_{t-1}(a) - C_t(a)$ . Additionally, if $b$ and $c$ are both $j$-th cousins, then the test $O^t_a(b,c)$ will not return a clear signal in either direction.
\end{lemma}
Note that $F^{t-1}_{t-1}(a) \subseteq F_{t-1}(a)$, and thus $L(T) - F^{t-1}_{t-1}(a) \subseteq L(T) - F_{t-1}(a)$. This means that the set of sinks in $G^t_a$ is exactly the set of $t$-th cousins of $a$. Also, oberve that if $e$ is in $F_{t-1}(a)$, then $e$ is also a $t$-th cousin of $b$, and by the above lemma, the entire $i-1$-th (true) family of $a$ will be matched as a $t$-th cousin of $b$ by the algorithm. Consider the case of a 


\end{comment}

For the induction step, we split the argument into multiple cases and steps within these cases. Let $F''_j(a)$ denote the $j$-th family of $a$ after the first phase of the algorithm.

\esh{The following lemmas are all claimed under the induction hypothesis on the invariants, reminder to point this out somewhere}

\begin{lemma}
\label{lemma:behave_alike}
If $a$ and $b$ are correctly connected in an earlier round (before round $t$), then, with high probability, if $O^t_c(b,d)$ returns an answer, then $O^t_c(a,d)$ returns the same answer, for all $c,d \notin F_{t-1}(a)$. Additionally, $O^t_a(b,c)$ does not (whp) returns $c$ for $c \notin F_{t-1}(a)$.
\end{lemma}

\begin{claim}
\label{claim:family_connections}
All connections $(a,b)$ made in the $t$-th round are made between $F^t_{t-1}(a)$ and $F^t_{t-1}(b)$.
\end{claim}

The analysis splits into two cases for any leaf $a$, depending on whether or not $a$ has a $t$-th cousin in the graph,i.e., whether $C_t(a) = \phi$.

First, we consider the case of when $C_t(a) \neq \phi$. The analysis proceeds in three steps.


\begin{lemma}
If $b$ is a $t$-th cousin of vertex $a$, then $a$ and $b$ are connected in the first phase. In fact, $F''_{t-1}(a)$ is connected to $F''_{t-1}(b)$.
\end{lemma}



\begin{lemma}
If $c \in F^{t-1}_{T-1}(a)$ was wrongly connected to $a$ in an earlier round, then $a$ and $c$ are disconnected in the first phase. If $c \in F^{t-1}_{T-1}(a)$ was correctly connected to $a$ in an earlier round, then $a$ and $c$ are not disconnected in the first phase. Taken together, $F''_{t-1}(a) = F_{t-1}(a)$.
\end{lemma}

\begin{lemma}
If $F''_{t-1}(a)$ is correctly connected to $F''_{t-1}(b)$ in the first phase, then the correct connection is retained at the end of the second phase. If $F''_{t-1}(a)$ is wrongly connected to $F''_{t-1}(c)$ in the first phase, then the correct connection is removed in the second phase. Also, $F^t_{t-1}(a) = F''_{t-1}(a)$.
\end{lemma}

Note that these three lemmas taken together guarantee the invariants for vertex $a$.

Now, consider the case of $a$ not having a $t$-th cousin, i.e., $C_t(a) = \phi$.

\begin{claim}
If $c \in F^{t-1}_{T-1}(a)$ was correctly connected to $a$ in an earlier round, then $a$ and $c$ are not disconnected in the first phase of the $t$-th round.
\end{claim}



The above claim suffices to prove the Invariant 1 for vertex $a$.

\input{proofs_full_trees}
\end{comment}

==> conclusions.tex <==
\label{sec:conclusions}
In this paper we have given a topology reconstruction under a very general model. We have also given a lower bound showing that reconstructing the topology is impossible if we weaken any of the assumptions made in our model. Thus, our results on topology reconstruction are the best possible. For weight reconstruction though, we have only given an algorithm for a specific function that determines the bias of the answers to queries. It is possible that we can do weight reconstruction for other specific functions as long as the function is known. It would be interesting to characterize the set of functions for which this is possible.

In the stochastic block model, we assume that we are given the entire graph generated stochastically based on community memberships of the vertices. Following this, we have assumed that the results of the entire set of $\genfrac(){0pt}{2}{n}{3}$ queries is given to us in our model. However, it would be interesting to try to optimize the number of queries needed for topology (and weight) reconstruction along the lines of \cite{kannan1996determining}.  We can show that for a very special case  where the unknown tree is a complete binary tree, all edges are of unit weight, and the bias probabilities follow our simple model, we can reconstruct the topology in $\tilde{O}(n)$ queries.
However, we leave a more thorough understanding of the query complexity for future work.

==> earlier_notes.tex <==
\section{Sufficient Conditions}
\subsection{First Approach - Simulating the Noisy Ultrametric Query Model}
\begin{lemma}
Every edge in the tree has weight $\frac{h(T)}{f(n)}$ where $f(n) = \frac{\sqrt{n}}{\log^2 n}$ ($h(T)$ is the height of the tree and and $n$ is the number of leaves).Under the assumption that the height of the tree is $O(\log n)$, this query model can be used to reconstruct, with probability at least $1-\frac{1}{poly(n)}$, the ``noisy ultrametric'' queries of \cite{kannan1996determining}, and hence to reconstruct the topology of the tree.
\end{lemma}

\esh{This lemma also has a bug similar to that in the proof of the next subsections's lemma}

%The template of the proof is as follows-  we will look at an arbitrary leaf triples $(a,b,c)$ and show that we can find simulate the noisy ultrametric query $U$, which returns the unique closest pair (since we are working with binary trees) with high probability (at least $1-\frac{1}{n^6}$). Then, we can use a union bound argument to argue that all $U(a,b,c)$ queries are correctly simulated with high probability.

%WLOG, let $d(a,b) < d(a,c) = d(b,c)$. To simulate $U(a,b,c)$ as $U'(a,b,c)$,  iterate over all leaves $x$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $f_x$ and $g_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ (respectively $(a,c)$). Let $F = \sum_x  f_x$ and $G = \sum_x g_x$. We decide $U'(a,b,c)$ based on comparing $F$ and $G$.

\subsection{Building a Partial Simulation of the Noisy Ultrametric Model}
We set up condtions under which we can partially reconstruct the noisy ultrametric queries oracle of \cite{kannan1996determining}, where an oracle $U$ takes a triple of leaves as the query and returns the closest pair. Given this oracle, \cite{kannan1996determining} comes up with an efficient algorithm to reconstruct the topology of the true. Let $N(a,b)$ represent the set of all leaves $l$ such that $d(a,l) \le d(a,b)$. Observe that $N(a,b) = N(b,a)$, consider any leaf $l$ such that $d(a,l) \le d(a,b)$, we know that either $l$ is closer to $a$ or $b$, in each case we can visually deduce from Figure~\ref{fig:neighbourhood} and~\ref{fig:nbhd2} that $l \in N(b,a)$. 
\begin{figure}[h]
    \centering
    \includegraphics[width =8cm]{images/neighbourhood.png}
    \caption{Case 1: Neighbourhood of $a,b$ - $N(a,b)$}
    \label{fig:neighbourhood}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width =8cm]{images/nbhd2.png}
    \caption{Case 2 : Neighbourhood of $a,b$ - $N(a,b)$}
    \label{fig:nbhd2}
\end{figure}

This neighbourhood $N(a,b)$ can be thought of as the set of all leaves ``between'' $a$ and $b$.

The partial oracle $U'$ has the following two properties $P_1$ and $P_2$:
\begin{itemize}
    \item When given queries of the form $(a,b,c)$ with $(a,b)$ as the closest pair, where $|N(a,b)| = o(\sqrt{n} \log n)$, and $c$ is a leaf such that $|N(a,c)| - |N(a,b)|  =  o(\sqrt{n} \log n)$, then $U'$ correctly returns the closest pair $(a,b)$. These conditions may seem somewhat contrived, but observe that a simple case that satisfies these conditions is when $a$ and $b$ are siblings, while $c$ is a first cousin of these two leaves. These conditions attempt to generalize the above case for sparser underlying tree topologies.
    \item When given queries of the form $(a,b,c)$ without the above properties, then the oracle either correctly returns the closest pair or does not return any answer.
\end{itemize}

\begin{lemma}
Every edge in the tree has weight $\frac{h(T)}{f(n)}$ where $f(n) = \frac{\sqrt{n}}{\log n}$ ($h(T)$ is the height of the tree and and $n$ is the number of leaves). Under these conditions, we can construct an oracle $U'$ that has properties $P_1$ and $P_2$ with high probability.
\end{lemma}

First, we describe the construction of the oracle $U'$. Given any leaf triple $(a,b,c)$, where, WLOG $d(a,b) < d(a,c) = d(b,c)$. Iterate over all leaves $x$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $f_x$ and $g_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ or $(b,x)$ (respectively $(a,c)$ or $(c,x)$). Let $F = \sum_x  f_x$ and $G = \sum_x g_x$. We decide $U'(a,b,c)$ based on comparing $F$ and $G$. Whenever we have $F \ge G + \kappa \sqrt{n} \log n$ ($\kappa$ is an appropriately chosen constant), or vice-versa, then we conclude that there is a ``strong'' signal and return $(a,b)$ (respectively $(a,c)$ if $G \ge F + \kappa \sqrt{n} \log n$). Otherwise, the oracle $U'$ does not return an answer.


Observe that both $F$ and $G$ are the sums of roughly $n$ independent $0-1$ random variables, therefore, it suffices to show that -
\begin{itemize}
    \item For property $P_1$, for the appropriate triples, the expectations of $F$ and $G$ are separated by $2\kappa \log n$.
    \item For property $P_2$, if $(a,b) < d(a,c) = d(b,c)$, then $\expect{F} \ge \expect{G}$ suffices to show that with high probability, an incorrect ``strong'' signal is not observed.
\end{itemize}

To complete the argument, the application of the Chernoff bound will show that $U'$ satisfies properties $P_1$ and $P_2$ in a ``pointwise'' sense, that is, for each triple $(a,b,c)$ with probability $1-\frac{1}{n^4}$. Therefore, using the union bound over all the possible $n^3$ many triples, we can say that the oracle satisfies the properties on all triples simultaneously with probability $1-\frac{1}{n}$.


\esh{Am unable to deal with a troublesome sub-case for proving property 2 pointwise}

Throughout the proof, we follow the convention that $d(a,b) < d(a,c) = d(b,c)$ and let $p$ be the LCA of $(a,b)$ while $q$ is the LCA of $(a,b,c)$.

To argue why property $P_1$ is satisfied- consider a triple $(a,b,c)$ satisfying the qualifying conditions i.e., let $d(a,b) < d(a,c) = d(b,c)$, and we have $|N(a,b)| = o(\sqrt{n} \log n)$; $|N(a,c)| - |N(a,b)|  =  o(\sqrt{n} \log n)$. Now, consider any leaves $x$ that is not present in the sub-tree rooted at $q$ (~Figure~\ref{fig:case1}). We know that there are $n -  o(\sqrt{n} \log n) = \theta(n)$ such leaves, and they are all the leaves in $L(T) - N(a,c)$.

\begin{figure}[h]
    \centering
    \includegraphics[width =8cm]{images/case1.png}
    %\caption{}
    \label{fig:case1}
\end{figure}
Now, getting to the numbers, let $d(a,b) = \alpha$, let $d(a,c) = d(b,c) = \beta$ and let $d(a,x) = d(b,x) = d(c,x) = \gamma$. Observe that $\alpha < \beta < \gamma$ and the differences are at least $2w$, where $w$ is the minimum weight of any edge in the tree.

Let $q$ represent the probability that $Q(a,b,x)$ returns either $(a,b)$ or $(b,x)$, while $q'$ represents the probability that $Q(a,c,x)$ returns either $(a,c)$ or $(c,x)$. We know that-
\[ q = \frac{2\gamma}{2(\alpha+2\gamma)} + \frac{\alpha + \gamma}{2(\alpha + 2\gamma)} = \frac{\alpha + 3 \gamma}{2(\alpha+2\gamma)} \]
A similar calculation yields - 
\[q' = \frac{\beta+3\gamma}{2(\beta + 2\gamma)} \]
Thus,
\begin{align*}
    \expect{f_x} - \expect{g_x} &= q-q'
    \\&= \frac{\alpha + 3 \gamma}{2(\alpha+2\gamma)} - \frac{\beta+3\gamma}{2(\beta + 2\gamma)}
    \\&=\frac{\gamma(\beta- \alpha)}{2(\alpha+2\gamma)(\beta+2\gamma)} 
    \\&\ge \frac{2w\gamma}{18\gamma^2}
    \\&\ge \frac{w}{9h(T)}
\end{align*}

Now, consider the random variables $F$ and $G$. We argue that $\expect{F} - \expect{G} \ge \kappa \sqrt{n} \log n$. Using linearity of expectation:
\[ \expect{F} - \expect{G} = \sum_{x \in L(T)} \expect{f(x)} - \expect{g(x)}\]
Splitting the leaves as within $N(a,c)$ and outside, we get -
\begin{align*}
    \expect{F} - \expect{G} &= \sum_{x \in N(a,c)} \expect{f(x)} - \expect{g(x)} + \sum_{x \notin N(a,c)} \expect{f(x)} - \expect{g(x)}
\end{align*}
By definition, we know that $|N(a,c)| = o(\sqrt{n} \log n)$, thus we can asymptotically lower bound (because it can be negative, which is detrimental to the cause) the first sum accordingly. Similarly, we know that $|L(T) - N(a,c)| = \theta(n)$. Therefore, we have-
\begin{align*}
    \expect{F} - \expect{G} &\ge -o(\sqrt{n \log n}) +\theta(n) \frac{w}{9 h(T)}
    \\&\ge \kappa \sqrt{n} \log n
\end{align*}

Here concludes the proof of property $P_1$.

Before proving property $P_2$, we establish a useful lemma about comparing the probabilities of certain outcomes of different queries.

\begin{lemma}
\label{lemma:monotone_comparison}
Consider the two queries $Q(a,b,x)$ and $Q(a,c,x)$. The, the inequality $\Pr[Q(a,b,x) = (a,x)] < \Pr[Q(a,c,x) = (a,x)]$ is true if and only if $d(a,b) + d(b,x) < d(a,c) + d(c,x) $.
\end{lemma}
The proof is directly seen by writing out the expressions for the respective probabilities.

Now, consider the case when $x \in N(a,b)$ (comparing $f_x$ and $g_x$), depicted by Figure~\ref{fig:case2}.
\begin{figure}[h]
    \centering
    \includegraphics[width = 8cm]{images/case2.png}
    \caption{}
    \label{fig:case2}
\end{figure}
In this case, we have $d(a,b) < d(a,c)$ and $d(b,x) < d(c,x)$, thus the conditions of Lemma~\ref{lemma:monotone_comparison} are satisfied, yielding $\expect{f_x} \ge \expect{g_x}$. More generally, this result also works when $d(a,b) < d(a,x) = d(b,x) < d(a,c) = d(c,x) = d(b,x)$.

\begin{note}
The above case can be shown to output a strong signal whp if each edge has weight $\Omega\left(\frac{h^2(T)}{\sqrt{n} \log n}\right)$, with the ``bad'' sub-case causing the quadratic height factor being that of the leaf $x$ satisfying $d(a,x) < d(a,b) = d(b,x)$.
\end{note}

\esh{The problem case}
%\esh{Potential fix -  accept some wrong strong signals, but prove that the above case will give a correct answer whp, rather than just never a wrong strong signal}

The final case is when  leaf $x$ satisfies $d(c,x) < d(a,c) = d(b,c)$, as depicted by Figure~\ref{fig:case3}.
\begin{figure}
    \centering
    \includegraphics[width=8cm]{images/case3.png}
    \caption{}
    \label{fig:case3}
\end{figure}

This case is somewhat problematic, because the comparison between $d(a,b) + d(b,x)$ and $d(a,c) + d(c,x)$ is decided by the comparison between $d(a,b)$ and $d(c,x)$, and can go in the wrong direction (as far as we are concerned) when $d(a,b) > d(c,x)$. In particular, the quantitatively bad case occurs when $d(a,b) >> d(c,x)$ and there are many such values of $x$, in which case our test might even end up generating a strong signal in the wrong direction.

\subsection{Limitation of the Partial Oracle}
We show an instance where the partial oracle will not suffice to exactly reconstruct the topology of the tree. Consider the instance shown by Figure~\ref{fig:bad_case}, where $B_{k}$ represents the balanced binary tree of height $k = \theta(\log n)$ (note that this height is possible under our conditions, which implicitly impose).

\begin{figure}
    \centering
    \includegraphics[width =8 cm]{images/bad_case.png}
    \caption{Bad Case for Partial Oracle}
    \label{fig:bad_case}
\end{figure}

Note that any triple containing either $a_1$ or $a_2$ might possibly always give an inconclusive result under our partial simulation of the noisy ultrametric query oracle. Therefore, it is impossible to distinguish between these two leaves just using the oracle $U'$.


\section{Summary of Findings so far}

First, a clarification about the partial oracle whose construction is attempted above. Note that finding the closest pair among three leaves $(a,b,c)$ implicitly finds the closer pair among $(a,b)$ and $(a,c)$. In fact, comparing $d(a,b)$ vs $d(a,c)$ and $d(a,b)$ vs $d(b,c)$ suffices to find the closest pair in $(a,b,c)$. Thus, we focus on a test that compares $d(a,b)$ and $d(a,c)$ (which can also deal successfully with the case where $d(a,b) = d(a,c)$.

The first test is what we call the ``obvious'' or O-test. Iterate over all leaves $x$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $h_x$ and $w_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ (respectively $(a,c)$). Let $H = \sum_x  h_x$ and $W = \sum_x w_x$. We decide $U'(a,b,c)$ based on comparing $H$ and $W$. Whenever we have $H \ge W + \kappa \sqrt{n} \log n$ ($\kappa$ is an appropriately chosen constant), or vice-versa, then we conclude that there is a ``strong'' signal and return $(a,b)$ (respectively $(a,c)$ if $W \ge H + \kappa \sqrt{n} \log n$). Otherwise, the oracle $U'$ does not return an answer.

The second test is called the adjusted test or A-test, since it accounts for discrepancies in the case where $x$ is close to $b$ (if $d(a,b) < d(a,c)$). Iterate over all leaves $x$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $f_x$ and $g_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ or $(b,x)$ (respectively $(a,c)$ or $(c,x)$). Let $F = \sum_x  f_x$ and $G = \sum_x g_x$. We decide $U'(a,b,c)$ based on comparing $F$ and $G$. Whenever we have $F \ge G + \kappa \sqrt{n} \log n$ ($\kappa$ is an appropriately chosen constant), or vice-versa, then we conclude that there is a ``strong'' signal and return $(a,b)$ (respectively $(a,c)$ if $G \ge F + \kappa \sqrt{n} \log n$). Otherwise, the oracle $U'$ does not return an answer.

For sake of analysis, we first focus on the case where $d(a,b) < d(a,c)$, similar ideas can be used in the case where $d(a,b) = d(b,c)$. The two tests give different signals depending on the relative positions of the leaves $x$.

We define a three-way partition for the comparison leaves $x$. Region $R_1$ is where $d(a,x) < d(a,b)$ or $d(a,b) < d(a,x) < d(c,x)$. Region $R_3$ is where $d(c,x) < d(a,c)$. Region $R_2$ is where $d(a,c) < d(a,x)$.

For $x \in R_1$, the O-test might signal in the wrong direction,i.e., $h_x < w_x$ is possible. The A-test signals in the right direction, with $\expect{f_x} - \expect{g_x} = \Omega(\frac{w_e}{h^2(T)})$.

For $x \in R_2$, the O-test signals in the right direction with $\expect{h_x} - \expect{w_x} = \Omega(\frac{w_e}{h(T)})$. The A-test might signal in the wrong direction.

For $x \in R_3$, both tests signal in the right direction, with an advantage of $\Omega(\frac{w_e}{h(T)})$.

Thus, when we are guaranteed that the number of leaves in $R_1$ and $R_2$ is $o(\sqrt{n} \log n)$, we can be sure of getting a strong correct signal. When this condition is violated for exactly one of $R_1$ or $R_2$, the corresponding test (A-test and O-test respectively) gives a signal in the right direction, with slightly stronger conditions needed for the A-test in the case of the condition violated for $R_1$. An open question is figuring out which is the ``right'' test since the wrong test can give a strong signal in the wrong direction. Finally, the case when the sparsity condition is violated for both $R_1$ and $R_2$ is also open, since we cannot tell which leaves $x$ come from which region.

==> general-model.tex <==
We can query any triple of leaves $(a,b,c)$ and get back one of the pairs $(a,b)$, $(b,c)$, or $(c,a)$ probabilistically.
Our probabilities should be such that it has a bias in favor of the closest pair. Recall that in an ultrametric, the other two pairs
are at the same distance. Thus we will model the probabilities of different answers as a function of just two distances --- $d_1$, the distance
between the closest pair of leaves and $d_2$ the distance between the two other pairs in the triple. (So $d_1 < d_2$. Equality is not possible
because we have a binary tree.) We also define two 
probabilities: $p_{\textsc{correct}}$ and $p_{\textsc{incorrect}}$ where $p_{\textsc{correct}}$ denotes the probability that the correct pair is
returned and $p_{\textsc{incorrect}}$ denotes the probability that one of the two incorrect pairs is returned. We assume that the two incorrect pairs
have an equal probability of being returned. Thus $\forall d_1, d_2, \ p_{\textsc{correct}}(d_1, d_2) + 2 p_{\textsc{incorrect}}(d_1, d_2) = 1$.
We require some mild conditions on these probability functions --- requiring that it be biased towards correct answers, and requiring an anti-Lipschitz condition that 
enforces that changes in the distances produce significant changes in probabilities.

\begin{enumerate}
\item $p_{\textsc{correct}} (d_1,d_2). \geq p_{\textsc{incorrect}} (d_1, d_2)$, $\forall 0 < d_1 < d_2$
\item For any fixed $d_2$ and $0 < d_1 < d_2$, $\frac{ \partial p_{\textsc{correct}}(d_1, d_2)}{\partial d_1}} \le -1$
\end{enumerate}

We could have imposed a similar partial derivative condition with respect to $d_2$, but this is not required for our results.

==> ideas.tex <==
1. Convex combination of weights (same topology) leads to a better weight
Start by expressing probabilities of the convex trees in terms of the the endpoints

Convexity- the one in the middle always performs better -implies unimodality



2.Hellinger - exact expression - also useful  - done

3. Top down for perfect trees, can get each edge down to $yn^-0.5$ - done, also $L_1$ error is significantly smaller than total edge weight. 

Extending this idea to unbalanced trees - something to do with centroid of a binary tree. root to centroid is well estimated, re-root at centroid (lose ultrametric?)

Look at figure in notes, Sampath's idea for 


4. Density of trees at different levels, for information theoretic tournament

5. 

==> intro.tex <==
\section{Introduction}

The problem of clustering elements based on some underlying notion of similarity is an important primitive that is used in multiple domains to learn the relationships between elements, and provide insights into the nature of the similarities between the elements of interest. In the standard clustering problem, a given set of elements is to be partitioned into subsets to minimize some objective based upon an underlying notion of distance between the elements. A natural and well studied generalization of this problem seeks to find a {\it hierarchical } partition of the elements, in which groups of elements form a nested structure. Canonical applications associated with this problem include learning evolutionary trees of a set of species and the evolutionary trees of languages. We will talk about the former problem in greater detail in the course of developing our model.

A critical aspect of any clustering problem is the exact formulation of the distance model and the method by which the algorithm is given access to this information. 


The problem of reconstructing evolutionary trees or phylogenies from data about extant species is an important one in computational biology~\cite{saitou1987neighbor, semple_steel_2003, farach1999efficient, Mossel_07_distorted_phylogeny, Kearney_97_soda, ailon2005fitting, Chor_quartets, daskalakis2006optimal, erdHos1999few, erdos1999few}. The specific formulation of the problem is defined by the type of data at the leaves and the objective function we seek to optimize. 

In the formulation~\cite{kannan1996determining} that is closest to the one in this paper, the evolutionary tree is assumed to be an \textit{ultrametric} binary tree, which is a weighted, rooted tree in which all root-leaf paths have the same length. This assumption is often justified in the computational biology literature based on the so-called molecular clock hypothesis, whereby the lengths of edges correspond to the evolutionary time that they represent. Then since all extant species are alive today and they are the leaves of this tree, they have all evolved for the same length of time. Hence all root-leaf paths have the same length. The model in \cite{kannan1996determining} assumes that we are able to perform experiments on any 3 extant species (leaves) $a,b,$ and $c$ and the result of the experiment is the pair that is closest together, i.e., has the most recent least common ancestor. In this model, the authors of \cite{kannan1996determining} give three different procedures for reconstructing the phylogeny that trade off running time against number of experiments. Several variants of this model have been explored subsequently~\cite{brown2013fast, Wy_phylogeny_2008}. 

In this paper we ask the question: What if the experiments are noisy? Since experiments on triples are typically based on stochastically generated data, our assumption that they are noisy is natural. Our main focus is on whether ultrametric trees can be reconstructed with noisy experiments, and we do not consider optimizing the number of experiments we perform. In this, we follow the setting of the stochastic block model (SBM), where there is an unknown partition of the vertices of a graph, and edges are generated stochastically with probabilities that depend on whether the two endpoints are in the same partition or not. In this model, it is commonly assumed that the entire graph is given, and the goal is to reconstruct the vertex partition.

We study a probability model where the probability of a particular pair being returned in an experiment on $a,b,$ and $c$ is purely a function of the three pairwise distances (two of which are equal because of ultrametricity).  The probability function must satisfy natural monotonicity conditions and Lipschitz conditions.  We show that we can reconstruct the topology of the tree with high probability in such a general model, given the results of all $\genfrac(){0pt}{2}{n}{3}$ experiments..

We also consider a more specific, simple model where the probabilities of each outcome are  specific simple functions of the distances. Perhaps somewhat surprisingly, we show that we can reconstruct not only the topology, but also the weights on the edges of the tree in this model described later, exploiting the functional dependencies of the probabilities on the edge weights. This is in contrast to the experiments in \cite{kannan1996determining} where there is simply no information for finding the weights.

The rest of the paper is organized as follows. In Section~\ref{sec:related} we review related work. In Section~\ref{sec:model} we precisely describe our models and problem statements. In Section~\ref{sec:topology} we design and analyze an algorithm for reconstructing the topology of the tree efficiently, given the answers to all $\genfrac(){0pt}{2}{n}{3}$ queries, under a fairly general noise model and with minimal assumptions about the edge weights. In Section~\ref{sec:weight} we give an algorithm for reconstructing edge weights under a specific noise model. In Section~\ref{sec:necessary}, we complement our algorithm for topology reconstruction, by showing that topology reconstruction cannot be guaranteed by any algorithm unless we have a condition on the minimum edge weight. Finally, in Section~\ref{sec:conclusions}, we highlight some directions for future work, including an insight into reducing the query complexity of topology reconstruction algorithms.

%Finally in Section~\ref{sec:query-optimal} we consider whether we can do the reconstruction with fewer than $n \choose 3$ queries and show that this can be done for a special case. We leave the problem of optimizing the number of queries for the general problem as an open question. \sk{Refer to a section on lower bounds here?}


\section{Related Work} \label{sec:related}

The problem of reconstructing evolutionary trees has received a lot of attention over the years. There are many formulations of this problem based on the type of data available and the objective function being optimized. Most formulations assume that the observed data is on extant species or leaves of an unknown tree. Objective functions seek to capture properties of the evolutionary process, with the hope that the optimal tree under an objective function is in fact the true evolutionary tree. The most popular formulations are distance-based methods~\cite{farachkannanwarnow,erdHos1999few, erdos1999few, saitou1987neighbor, mossel2017distance, daskalakis2013alignment} (where we are given a matrix of distances between leaves and we want to find the best-fitting edge-weighted tree), character-based methods~\cite{agarwalaf-b,kannanwarnow,mossel2005learning, MosselS07, steel2016phylogeny}, where we want to explain the evolution of different characters, each taking on a state in each extant species using the fewest number of state changes, and likelihood methods~\cite{neyman1971molecular, felsenstein1981evolutionary,farach1999efficient, roch2017phase}, where we assume that evolution is a stochastic process drawn from a family of processes, and want to estimate the most likely parameters. In all cases the data observed at the leaves is the result of the stochastic process of evolution. These formulations and other related types lend themselves naturally to the model considered in this paper. 


The current paper is also related to the rich line of  work on the so-called stochastic block model (SBM)\cite{mcsherry2001spectral, mossel2018proof, decelle2011asymptotic, abbe2017community}.  In SBM, the goal is to discover an underlying partition of the set of vertices into two (or more) unknown clusters. The algorithm gets to query pairs $(i,j)$ of vertices and gets an edge (i) with probability $p$ if $i$ and $j$ belong to the same cluster; (ii) with probability $q<p$ if $i$ and $j$ belong to different clusters.  After making all $\genfrac(){0pt}{2}{n}{2}$ queries, we want to `reconstruct' the clusters. There are several notions of what it means to reconstruct, and which ones are achievable depending on the relative values of $p$ and $q$. The current work differs from the line of work on SBM in two ways: (i) Instead of queries on pairs, we allow for queries on triples of vertices. (ii) Our goal can be construed as recovering a {\em hierarchical cluster} -- as opposed to the {\em flat clusters} in the SBM model. 



%We can think of the goal here as discovering an underlying  partition of  We can query a pair of vertices to ascertain if there is an edge between them. For a pair $(i,j)$, if $i$ and $j$ are in the same cluster, there is an edge between them with probability $p$, whereas if they are in different clusters, this probability is $q < p$. 

Another variant of the SBM which is related to the current paper is the work of Chen et al.\cite{chen2020near}. Here, the vertices lie in a metric space, rather than being just members of some cluster. The probability of an edge between two vertices is a function of their distance. The goal is to observe a graph generated with these edge probabilities, and infer the (approximate) positions of the vertices. %\cite{chen2020near} shows that for the Euclidean space in one or two dimensions, where edge probabilities decay as a nice function of the distance, as long as we have a dense enough set of vertices, we can efficiently locate them at approximately their correct positions. 
Chen et al.~\cite{chen2020near} show that for the Euclidean space in one or two dimensions, where edge probabilities decay as a nice function of the distance, a dense enough set of vertices can be efficiently located at approximately their correct positions. 
In the 1-D case we can find the approximate order among the vertices even more efficiently. These results are shown for edge probabilities that are inverse-exponential, or inverse polynomial in the distance. %{\tempcol{Note that in contrast to \cite{chen2020near} where the points lie in $\mathbb{R}^d$, in the current paper, the points lie on an ultrametric.}}
Note that in contrast to \cite{chen2020near} where the points lie in $\mathbb{R}^d$, in the current paper, the points lie on an ultrametric.





==> intro_old.tex <==
\section{Introduction}

The problem of reconstructing evolutionary trees or phylogenies from data about extant species is an important one in computational biology~\cite{saitou1987neighbor, semple_steel_2003, farach1999efficient, Mossel_07_distorted_phylogeny, Kearney_97_soda, ailon2005fitting, Chor_quartets, daskalakis2006optimal, erdHos1999few, erdos1999few}. The specific formulation of the problem is defined by the type of data at the leaves and the objective function we seek to optimize. 

In the formulation~\cite{kannan1996determining} that is closest to the one in this paper, the evolutionary tree is assumed to be an \textit{ultrametric} binary tree, which is a weighted, rooted tree in which all root-leaf paths have the same length. This assumption is often justified in the computational biology literature based on the so-called molecular clock hypothesis, whereby the lengths of edges correspond to the evolutionary time that they represent. Then since all extant species are alive today and they are the leaves of this tree, they have all evolved for the same length of time. Hence all root-leaf paths have the same length. The model in \cite{kannan1996determining} assumes that we are able to perform experiments on any 3 extant species (leaves) $a,b,$ and $c$ and the result of the experiment is the pair that is closest together, i.e., has the most recent least common ancestor. In this model, the authors of \cite{kannan1996determining} give three different procedures for reconstructing the phylogeny that trade off running time against number of experiments. Several variants of this model have been explored subsequently~\cite{brown2013fast, Wy_phylogeny_2008}. 

In this paper we ask the question: What if the experiments are noisy? Since experiments on triples are typically based on stochastically generated data, our assumption that they are noisy is natural. Our main focus is on whether ultrametric trees can be reconstructed with noisy experiments, and we do not consider optimizing the number of experiments we perform. In this, we follow the setting of the stochastic block model (SBM), where there is an unknown partition of the vertices of a graph, and edges are generated stochastically with probabilities that depend on whether the two endpoints are in the same partition or not. In this model, it is commonly assumed that the entire graph is given, and the goal is to reconstruct the vertex partition.

We study a probability model where the probability of a particular pair being returned in an experiment on $a,b,$ and $c$ is purely a function of the three pairwise distances (two of which are equal because of ultrametricity).  The probability function must satisfy natural monotonicity conditions and Lipschitz conditions.  We show that we can reconstruct the topology of the tree with high probability in such a general model, given the results of all $\genfrac(){0pt}{2}{n}{3}$ experiments..

We also consider a more specific, simple model where the probabilities of each outcome are  specific simple functions of the distances. Perhaps somewhat surprisingly, we show that we can reconstruct not only the topology, but also the weights on the edges of the tree in this model described later, exploiting the functional dependencies of the probabilities on the edge weights. This is in contrast to the experiments in \cite{kannan1996determining} where there is simply no information for finding the weights.

The rest of the paper is organized as follows. In Section~\ref{sec:related} we review related work. In Section~\ref{sec:model} we precisely describe our models and problem statements. In Section~\ref{sec:topology} we design and analyze an algorithm for reconstructing the topology of the tree efficiently, given the answers to all $\genfrac(){0pt}{2}{n}{3}$ queries, under a fairly general noise model and with minimal assumptions about the edge weights. In Section~\ref{sec:weight} we give an algorithm for reconstructing edge weights under a specific noise model. In Section~\ref{sec:necessary}, we complement our algorithm for topology reconstruction, by showing that topology reconstruction cannot be guaranteed by any algorithm unless we have a condition on the minimum edge weight. Finally, in Section~\ref{sec:conclusions}, we highlight some directions for future work, including an insight into reducing the query complexity of topology reconstruction algorithms.

%Finally in Section~\ref{sec:query-optimal} we consider whether we can do the reconstruction with fewer than $n \choose 3$ queries and show that this can be done for a special case. We leave the problem of optimizing the number of queries for the general problem as an open question. \sk{Refer to a section on lower bounds here?}


\section{Related Work} \label{sec:related}

The problem of reconstructing evolutionary trees has received a lot of attention over the years. There are many formulations of this problem based on the type of data available and the objective function being optimized. Most formulations assume that the observed data is on extant species or leaves of an unknown tree. Objective functions seek to capture properties of the evolutionary process, with the hope that the optimal tree under an objective function is in fact the true evolutionary tree. The most popular formulations are distance-based methods~\cite{farachkannanwarnow,erdHos1999few, erdos1999few, saitou1987neighbor, mossel2017distance, daskalakis2013alignment} (where we are given a matrix of distances between leaves and we want to find the best-fitting edge-weighted tree), character-based methods~\cite{agarwalaf-b,kannanwarnow,mossel2005learning, MosselS07, steel2016phylogeny}, where we want to explain the evolution of different characters, each taking on a state in each extant species using the fewest number of state changes, and likelihood methods~\cite{neyman1971molecular, felsenstein1981evolutionary,farach1999efficient, roch2017phase}, where we assume that evolution is a stochastic process drawn from a family of processes, and want to estimate the most likely parameters. In all cases the data observed at the leaves is the result of the stochastic process of evolution. These formulations and other related types lend themselves naturally to the model considered in this paper. 


The current paper is also related to the rich line of  work on the so-called stochastic block model (SBM)\cite{mcsherry2001spectral, mossel2018proof, decelle2011asymptotic, abbe2017community}.  In SBM, the goal is to discover an underlying partition of the set of vertices into two (or more) unknown clusters. The algorithm gets to query pairs $(i,j)$ of vertices and gets an edge (i) with probability $p$ if $i$ and $j$ belong to the same cluster; (ii) with probability $q<p$ if $i$ and $j$ belong to different clusters.  After making all $\genfrac(){0pt}{2}{n}{2}$ queries, we want to `reconstruct' the clusters. There are several notions of what it means to reconstruct, and which ones are achievable depending on the relative values of $p$ and $q$. The current work differs from the line of work on SBM in two ways: (i) Instead of queries on pairs, we allow for queries on triples of vertices. (ii) Our goal can be construed as recovering a {\em hierarchical cluster} -- as opposed to the {\em flat clusters} in the SBM model. 



%We can think of the goal here as discovering an underlying  partition of  We can query a pair of vertices to ascertain if there is an edge between them. For a pair $(i,j)$, if $i$ and $j$ are in the same cluster, there is an edge between them with probability $p$, whereas if they are in different clusters, this probability is $q < p$. 

Another variant of the SBM which is related to the current paper is the work of Chen et al.\cite{chen2020near}. Here, the vertices lie in a metric space, rather than being just members of some cluster. The probability of an edge between two vertices is a function of their distance. The goal is to observe a graph generated with these edge probabilities, and infer the (approximate) positions of the vertices. %\cite{chen2020near} shows that for the Euclidean space in one or two dimensions, where edge probabilities decay as a nice function of the distance, as long as we have a dense enough set of vertices, we can efficiently locate them at approximately their correct positions. 
Chen et al.~\cite{chen2020near} show that for the Euclidean space in one or two dimensions, where edge probabilities decay as a nice function of the distance, a dense enough set of vertices can be efficiently located at approximately their correct positions. 
In the 1-D case we can find the approximate order among the vertices even more efficiently. These results are shown for edge probabilities that are inverse-exponential, or inverse polynomial in the distance. %{\tempcol{Note that in contrast to \cite{chen2020near} where the points lie in $\mathbb{R}^d$, in the current paper, the points lie on an ultrametric.}}
Note that in contrast to \cite{chen2020near} where the points lie in $\mathbb{R}^d$, in the current paper, the points lie on an ultrametric.





==> notation_old.tex <==
\section{Model, Notation, and Preliminaries} \label{sec:model}
There is an underlying weighted tree $T$ with the weights constrained such that the distance function between leaves is an ultrametric. The set of leaves of the tree is represented by $L(T)$.  We assume that the height of the tree $h(T)$ is normalized to $1$.

{\bf General  Model:} For each triple of leaves $(a,b,c)$, we perform an experiment (query) and get back one of the pairs $(a,b)$, $(b,c)$, or $(c,a)$ probabilistically. Such an experiment will be denoted by $Q(a,b,c)$.
Recall that in an ultrametric, the top two of the three pairwise distances are equal.
Thus we will model the probabilities of different answers as a function of just two distances --- $d_1$, the distance
between the closest pair of leaves and $d_2$ the distance between either of the two other pairs in the triple. (So $d_1 < d_2$. Equality is not possible
because we have a binary tree.) We also define two 
probabilities: $p_{\textsc{correct}}$ and $p_{\textsc{incorrect}}$ where $p_{\textsc{correct}}$ denotes the probability that the correct pair is
returned and $p_{\textsc{incorrect}}$ denotes the probability that one of the two incorrect pairs is returned. In our model, the two incorrect pairs
have equal probabilities of being returned. Thus $\forall d_1, d_2, \ p_{\textsc{correct}}(d_1, d_2) + 2 p_{\textsc{incorrect}}(d_1, d_2) = 1$.
We require some mild conditions on these probability functions --- requiring that they be biased towards correct answers, and requiring an anti-Lipschitz condition that 
enforces that significant changes in distances produce significant changes in probabilities.

\begin{enumerate}
\item $p_{\textsc{correct}} (d_1,d_2) \geq p_{\textsc{incorrect}} (d_1, d_2)$, $\forall \ 0 < d_1 < d_2$
\item For any $d_2$ and $0 < d_1 < d_2$, $\frac{ \partial p_{\textsc{correct}}(d_1, d_2)}{\partial d_1} \le -\varepsilon$, for some constant $\varepsilon  > 0$.
\item As $d_1 \rightarrow d_2$, we have $p_{\textsc{correct}} (d_1,d_2) \rightarrow 1/3$.
\end{enumerate}


Repeating an experiment produces the same answer, and results of distinct experiments are independent of each other.  We will refer to this model as the \textbf{general model}. 

When it comes to reconstructing weights (Section~\ref{sec:weight}), we show that it is possible for a specific instantiation of this general model, called the \textbf{simple model}, described below.


%Next, we describe the \textbf{simple model} which is a specific instantiation of the \textbf{general model}. In particular, while the results in Section 4 hold for the general model, our results in Section are only for the simple model

Here  an experiment on leaves $(a,b,c)$, outputs the pair  $(a,b)$ with probability $\frac{d(a,c) + d(b,c)}{2(d(a,b) +d(a,c) + d(b,c))}$.  If $d(a,b)$ is the smallest of the 3 pairwise distances, then the probability of the query returning $(a,b)$ is between 1/3 and 1/2. Since  the other two distances, $d(a,c)$ and $d(b,c)$ are equal in an ultrametric,  the query has equal probability of returning $(a,c)$ or $(b,c)$.  
Thus for pairs $a, b$ that are very close and $c$ that is much farther, the probability of getting the result $(a,b)$ approaches .5, while for triples $(a,b,c)$ whose least common ancestors are really close, the probability of getting any pair approaches $1/3$. 

%Note that the simple model satisfies the  properties of the general model with the partial derivative (of the probability of getting a correct answer with respect to the smallest distance) being at least $\frac{1}{6}$ in magnitude, rather than the magnitude being at least $1$. 

Even in the simple model, we cannot hope to reconstruct arbitrary ultrametrics as the following example shows: the underlying tree is a balanced binary tree, with each edge at depth $i$ having weight $2^i$ (the weights can be thought of as normalized through dividing by the total weight of the root to leaf path).  Let $h$ be the height of the tree. Consider any 3 leaves all of whose least common ancestors are in the top $\log n / 2$ layers. It is clear that the pair with the lowest least common ancestor has negligible advantage over the other two pairs. For any 3 such leaves, $a,b,$ and $c$, and for any other leaves $x$ and $y$,
it can be checked that any experiment involving two of $a,b,$ and $c$ and $x$  has indistinguishable probability of producing each of the 3 results, regardless of which pair out of $a,b,$ and $c$ is used in the experiment. Similarly any experiment involving  $x$ and $y$ and one of $a,b,$ and $c$ has indistinguishable probability of producing $(x,y)$ regardless of which of $a,b,$ or $c$ is used. Thus, with only $n^3$ experiments and negligible advantage from each, it will be impossible to learn even partial information about the topology in the top half of the tree. 

Thus, we will need to impose some conditions on the ultrametric to make the problem tractable. 

\subsection{Our Results}
\begin{enumerate}
\item We give an efficient algorithm that, with high probability, exactly reconstructs any ultrametric binary tree in the general model, under the condition that the length of each edge is at least $\tau \fs$.(Theorem~\ref{theorem:topology}). 
\item We complement the above result by showing that there exists no algorithm to reconstruct the topology of  trees with edge weights smaller than $\frac{1}{100\sqrt{n}}$  (Theorem~\ref{theorem:necessary}). 
\item Finally, we give an efficient algorithm that reconstructs the edge weights with high probability up to additive error $\kappa \frac{\log n}{\sqrt{n}}$ assuming each edge weight is at least $\tau  \frac{\log n}{\sqrt{n}}$ (Theorem~\ref{theorem:weights}) in the simple model. (Remark: We present our result assuming that the topology of the tree is already known, but since this model is a special case of the general model, we can also first reconstruct the topology of the tree before finding the weights.)
\end{enumerate}

Again, wlog, we will assume that our trees are full, since an internal node with 1 child does not affect the response to any query and can be eliminated. 
%\begin{note}
Through this paper, when we refer to events having \ohp, we mean a probability of at least $1- \frac{1}{n^6}$. 
%\end{note}

Since we will consider at most $o(n^5)$ such events, using the union bound, we can assume that all of them happen with very high probability (at least $1-\frac{1}{n}$), and condition our analysis upon this event.% All probabilities are taken purely over the randomness in the ${n \choose 3}$ possible queries. In the analysis of our algorithms, we chain together a sequence of random events $F_1, F_2, \cdots $ by proving that each conditional probability $\Pr[F_i | F_1, F_2 \cdots F_{i-1}]$ is sufficiently large and using the union bound.




\subsection{Notation for Trees}
We fix some standard notation for full binary trees that will be used in our algorithms.


{\bf Subtrees: } By  a \textit{subtree} of some tree $T$, we will mean the entire tree rooted at some internal node of $T$. (Thus we use the term ``subtree'' in a more restrictive manner than usual.) For any tree $T$, $L(T)$ denotes the set of leaves of $T$. We will also refer to the set of all leaves in the tree by $L$. 
%\esh{We need a different description, will come back to this after the reconstruction algorithm is stable}

{\bf Subtree Induced Partition:} If $T_B$ is a subtree of $T$, it naturally partitions $L(T) - L(T_B)$ into buckets $S_1, S_2, \cdots S_k$ , where $x$ and $y$ are in the same bucket if and only if for any $z \in L(T_B)$, the least common ancestors of $x$ and $z$, and of $y$ and $z$ are the same. An alternative characterization of these buckets is that $x$ and $y$ are in the same bucket if and only if for any $z$ in $T_B$, the closest pair out of the triple $(x,y,z)$ is $(x,y)$.  Each bucket can be thought of as a subtree hanging off from the path from the root of $T_B$ to the root of $T$. Thus there is a natural order on the buckets that is defined by this path, with $S_1$ being the bucket closest to $T_B$ and $S_k$ be the farthest. 
A visual depiction is shown in Figure~\ref{fig:total_order}.  For any $j \in [k]$, the set of leaves in $T_B, S_1, S_2 \cdots S_j$ form the leaves of a subtree.
%\sk{Hid the figure... could be put back.  Removed mention of strict weak order... need to remove it everywhere else.}
%\esh{Have put it back}

{\bf Induced Topology:}   For any subset of leaves $S$ we can define the induced topology on $S$ by removing all leaves outside of $S$ and getting rid of internal nodes that now have only one child. (Since we are talking about weighted trees, when we have an internal node $v$ with one child, we replace the two edges incident on $v$ by a single edge whose weight is the sum of the weights of the two edges.)  It is not hard to see that the weighted tree obtained by this process will define an ultrametric on $S$. As a special case, when $T_B$ is a subtree of $T$, we will denote the induced topology on the leaves \textbf{not} in $T_B$ by $T - T_B$.
We will also define a slightly different induced topology where we replace $T_B$ by a single leaf (of $T_B$). We think of this operation as taking the quotient of $T$ with respect to $T_B$, and denote the resulting topology by $T\, / \, T_B$. 


By the \textit{topology of a triple} of leaves $(x,y,z)$ we mean the induced subtree of $T$ with just these leaves. This topology is completely specified by specifying the pair among $x,y,$ and $z$ that has the least common ancestor of smallest height.

Finally, we use some standard concentration inequalities and  results about measures of statistical distance in our paper. These can be found in Appendix~\ref{sec:con}.




\begin{figure}[h]
    \centering
    \includegraphics[width = 6cm]{new_images/bucket_partition.png}
    \caption{Partition of buckets with respect to Subtree $T_B$}	
    \label{fig:total_order}
\end{figure}



==> old content/old_full_trees.tex <==


Our algorithm locally reconstructs the tree bottom up, adding new connections in each round. New connections are made exclusively by the process of introducing a new internal vertex and setting two disjoint subtrees to be its children.

Let $T'$ $C',F'$ represent the forest, the cousin relation and the family relations as maintained by the algorithm. At the beginning, $T'$ is a union of $n$ singleton trees, where each tree is a unique leaf in $L(T)$. The cousin and forest relations are initialized to be null sets. Define $F'(a) = \cup_{i \in [n] \cup \{0,-1\}} C'_i(a)$. Alternatively, $F'(a)$ can be understood to be all leaves reachable from $a'$ in the forest $T'$. We overload the notation and also let $F'(a)$ denote the sub-tree containing all the leaves in $F'(a)$. The algorithm also maintains a set of meta-leaves $ML(T')$, such that every leaf in a family $F'(a)$ is represented by a single leaf (of the family) in the set $ML(T')$. At the start of the algorithm, for every leaf $F'(a) = a$ and the set of meta-leaves is exactly the set of all leaves of the tree. Intuitively, the meta leaves represent connected subtrees, at the beginning each leaf is a connected subtree and at the end, the entire tree is the only connected subtree. 


\subsection{The Algorithm}
The algorithm proceeds in rounds, and each round has two parts. %First, we sketch the sub-procedures used in both parts.

The following sub-procedure sketches the method used to extend a large family $F'(a)$ that satisfies the property that $|F'(a)| \ge \frac{n}{3}$.

{	
\begin{algorithm}[ht]
	{
		\label{algorithm:large_familie}
			\caption{Algorithm for Extending a Large Family $F'(a)$}
		\begin{algorithmic}[1]
		%\STATE x=5
		\STATE Consider all pairs $b,c \in ML(T')  - \{a\}$. $ b$  is considered to win over $c$  if there are $\kappa \sqrt{n \log n}$ more $(x,b)$ answers than $(x,c)$ answers over all $(x,b,c)$ queries for $x \in F'(a)$. The same rule is used to decide if $c$ is the winner. (It is possible that there is no winner). Here $\kappa = 30$.
		\STATE Draw the tournament graph with vertices $ML(T')  - \{a\}$. Draw an edge from $b$ to $c$ if $c$ wins over $b$. If this graph has a unique sink $s$, then connect the families $F'(a)$ and $F'(s)$. Remove $s$ from the set of meta leaves $ML(T')$. Set all leaves in $F'(a)$ to be part of the meta leaf $a$. Reroot the subtree containing $a$ at the new internal vertex added in this step.
		\end{algorithmic}
    }
	\end{algorithm}
}		

We now describe each round of the algorithm, which is run until all leaves are connected. The algorithm also keeps tracking of a rooting of the disjoint subtrees of $T'$.

 
{	
\begin{algorithm}[ht]
\label{algorithm:round_algorithm}
			\caption{Algorithm for each Round}
	{
		
		\begin{algorithmic}[1]
		%\STATE x=5
		\STATE While there are leaves $a \in ML(T')$ such that $|F'(a)| \ge \frac{n}{3}$, run Algorithm~\ref{algorithm:large_familie} on family $F'(a)$. Repeat until there is no more progress.
	    \STATE Consider all pairs $a,b \in ML(T')$ such that $|F'(a)|, |F'(b)| <  \frac{n}{3}$. Each pair is assigned a score $s_{a,b}$ which is the average number of $(a,b,x)$ queries that return $(a,b)$ over all $x \in L(T) - (F'(a) \cup F'(b))$.
	    \STATE Connect $F'(a)$ and $F'(b)$ for the highest scoring pair (breaking ties arbitrarily). Remove $b$ from the set of meta-nodes $ML(T')$. Set all leaves in $F'(a)$ to be part of the meta leaf $a$. Reroot the subtree containing $a$ at the new internal vertex added in this step.
		\end{algorithmic}
    }
	\end{algorithm}
}		

Note that connecting two families $F'(a)$ and $F'(b)$ is done by introducing a new internal node (corresponding to the least common ancestor of $a$ and $b$) and making the two trees children of this node.

The overall algorithm keeps invoking Algorithm~\ref{algorithm:round_algorithm} until all the leaves are connected in the forest $T'$,i.e., until $T'$ becomes a tree.


We claim that the algorithm maintains the following invariants at the end of each round.

\begin{lemma}
\label{lemma:invariants}
Let $T'$ be the forest maintained by the algorithm at the end of some round, with meta leaves $ML(T')$ and implicit cousin and family relationships denoted by $C'$ and $F'$. $T'$ has the following properties (essentially, invariants maintained by the algorithm) -

\begin{enumerate}
    \item $T'$ is a union of disjoint full binary trees and these trees are rooted so that $L(T') = L(T)$. Here $L(T')$ is the union of the leaf sets of all the disjoint subtrees of $T$.
    \item $C'$ and $F'$ are symmetric relationships. In fact, $C'$ and $F'$ are generated by examining $T'$, which makes them symmetric by construction.
    \item $a \in C'_i(b)$ implies that for all indices $j \le i$, we have both $C'_j(a) = C_j(a)$ and $C'_j(b) = C_j(b)$. Equivalently, for any leaf $a$, the tree denoted by $F'(a)$ is equivalent to a $\sst$ t of $T$ containing the leaf $a$.
    \item $a \in F'(b)$ if and only if $ML(a) = ML(b)$, i.e., two connected leaves are represented by the same meta-leaf.
\end{enumerate}
\end{lemma}


The following lemma guarantees progress in each round.

\begin{lemma}
\label{lemma:progress}
At least one new vertex is added to the forest $T'$ in each round and no vertices are removed. 
\end{lemma}

As an immediate corollary of the above two lemmas:

\begin{corollary}
\label{corollary:progress}
Let $C''$ represent the cousin relationship before a round, and $C'$ the cousin relationship after. ,
\begin{enumerate}
    \item $\exists$ leaf $a$ and index $i$ such that $C''_i(a) = \phi $ and $C_i'(a) \neq \phi$.
    \item $\forall a \in L(T)$, $\forall i$: $C_i''(a) \subseteq C_i'(a)$.
\end{enumerate}
\end{corollary}





\subsection{Proof of Correctness}

To begin, we show that the algorithm terminates after a polynomial number of rounds and perfectly reconstructs the tree given that Lemmas~\ref{lemma:invariants} and~\ref{lemma:progress} are true.
Lemma~\ref{lemma:progress} indicates that at least two leaves that were not connected in the forest $T'$ at the beginning of a round are connected by the end (by adding a new internal vertex) of this round.

The following two lemmas are elementary properties of trees.

\begin{lemma}
A full binary tree with $n$ leaves has exactly $n-1$ internal vertices.
\end{lemma}

\begin{lemma}
A forest that is a disjoint union of $k$ binary trees, each rooted so that there are $n$ leaves in total has $n - k$ internal vertices.
\end{lemma}

Observe that Lemmas~\ref{lemma:invariants} and~\ref{lemma:progress} indicate that each round decreases the number of disjoint subtrees by at least $1$, since each new vertex added connects two disjoint full subtrees. Initially, there are $n$ disjoint full subtrees, and the algorithm terminates when there is only $1$ full subtree. Consequently, the algorithm runs for at most $n-1$ rounds.


The proof is complete if we can prove Lemmas~\ref{lemma:invariants} and~\ref{lemma:progress}.


\subsection{Proof of Lemmas~\ref{lemma:invariants} and~\ref{lemma:progress}}
We prove Lemma~\ref{lemma:invariants} using induction. Trivially, the initialization of $T', C'$ and $F'$ satisfies the conditions. Assuming they hold at the end of the $k$-th round, we show that they will hold at the end of the $k+1$-th round. 

\subsubsection{Correctness of Algorithm~\ref{algorithm:large_familie}}
First, we will show that running Algorithm~\ref{algorithm:large_familie} preserves the invariants. Consider a leaf $a \in ML(T')$ with $|F'(a)| \ge \frac{n}{3}$ that is considered by the algorithm. Let us consider the subtree rooted at vertex $v_a$ denoted implicitly by $F'(a)$. Since the algorithm has not yet terminated, there are other subtrees in the forest $T'$, indexed by $ML(T') - \{a\}$. 



Using the induction hypothesis, for every meta leaf $l \in ML(T')$, we know that the subtree $F'(l)$ is equivalent to a $\sst$  of the original tree $T$ - let us index this subtree as $T_l$.  Let vertex $v$ be the internal vertex in $T$ that is a parent of $T_a$ (we know that such a vertex exists because if $T_a = T$, the algorithm would have terminated since all leaves would have been connected). Let $T^*$ be the $\sst$ t of $T$ rooted at the other child of vertex $v$. 

\begin{claim}
\label{claim:large_winner}
Let $b \in ML(T') -\{a\}$ be a meta-leaf contained in $T^*$ and let $l \in ML(T') - \{a\}$ be a meta-leaf not contained in the $\sst$ rooted at vertex $v$. Then, with overwhelmingly high probability, $b$ wins over $l$.
\end{claim}

\begin{proof}
We know that $T_a$, $T_{b}$ and $T_{l}$ are all disjoint, since $a,b$ and $l$ are disconnected leaves in $T'$.Further, we can conclude that on the original tree $T$, $d_1 := d(x,b) < d(x,l) = d(b,l) =: d_2$ for all leaves $x \in L(T_a) = F'(a)$ -this can also be inferred from Figure~\ref{fig:comparisonwinner_alg1}. Let $x_1,x_2,..x_k$ represent the leaves in $F'(a)$ (with $k \ge \frac{n}{3}$). Let $Y_1, Y_2,..Y_k$ represent the random variables that query $Q(x_i,b,l)$ returns $(x_i,b)$ as the closest pair. Observe that these $\{Y_i\}$s are i.i.d. random variables, each with mean $\frac{2d_2}{2(2d_2 + d_1)}$. Let their realizations be $y_1,y_2,..y_k$. Let $Z_1,Z_2,..Z_k$ represent the random variables that query $Q(x_i,b,l)$ returns $(x_i,l)$ as the closest pair. These $\{Z_i\}$s are i.i.d. random variables, each with mean $\frac{d_1 + d_2}{2(2d_2 + d_1)}$. Let their realizations be $z_1,z_2,..z_k$. Let $Y = \sum_{i=1}^k y_i$ and $Z = \sum_{i=1}^k z_i$. Observe that $\E[Y] - \E[Z] = \frac{d_2 - d_1}{2(2d_2 +d_1)} \ge \frac{  \tau}{6} \fs %\ge \frac{\tau \sqrt{n \log n} }{18} 
$, based on the conditions we have assumed about the minimum weight of any edge (since the length of the path from $x$ to $l$ is greater than the length of the path from $x$ to $b$ plus the weight of at least one edge in the tree). 

\begin{figure}[h]
    \centering
    \includegraphics[width=10cm]{images/lemma invariants/comparison.png}
    \caption{Relative Arrangement of $x,b$ and $l$}
    \label{fig:comparisonwinner_alg1}
\end{figure}

\begin{claim}
With probability at least $1 - \frac{1}{n^6}$, $Y > Z + \kappa \sqrt{n \log n}$.
\end{claim}

\begin{proof}

Note that $\E[Y] - E[Z] \ge \frac{\tau}{} \sqrt{n \log n}$, using the condition for minimum weight of an edge.
Let $T$ be the midpoint between $\E[Y]$ and $\E[Z] + \frac{\tau}{6} \sqrt{n \log n}$. 
For sufficiently large constant $\tau$ \esh{add specific value}, by the Chernoff bound, we know that the events $Y > T + \frac{\tau}{24} \sqrt{n \log n}$ and $Z < T$ happen with probability at least $1 - \frac{1}{2n^6}$ respectively. An application of the union bound gives that result that $Y >  Z + \kappa \sqrt{n \log n}$ with the desired probability lower bound.
\end{proof}

This concludes the proof that $b$ almost surely wins over $l$.
\end{proof}


\begin{claim}
\label{claim:no_winner}
Let $b_1, b_2 \in ML(T') - \{a\}$ be two meta-leaves contained in the tree $T^*$. Then, with overwhelmingly high probability, there is no winner in this contest.
\end{claim}

\begin{proof}
We know that $T_a$, $T_{b_1}$ and $T_{b_2}$ are all disjoint, since $a,b_1$ and $b_2$ are disconnected leaves in $T'$. Thus, we can conclude that on the original tree $T$, $d(b_1,b_2) < d(x,b_1) = d(x,b_2)$ for all leaves $x \in L(T_a) = F'(a)$. This can be inferred from Figure~\ref{fig:nowinner}, where it is clear that the path from $x$ to $b_1$ (or $b_2$) contains (strictly) half the path (lengthwise) from $b_1$ to $b_2$.


\begin{figure}[h]
    \centering
    \includegraphics[width=10cm]{images/lemma invariants/nowinner.png}
    \caption{Relative Arrangement of $x,b_1$ and $b_2$}
    \label{fig:nowinner}
\end{figure}

%fse
%//////
In particular, using the condition on minimum edge weights : $d(x,b_1) + \tau \fs  \le d(x,b_1) = d(x,b_2)$. Let $x_1,x_2...x_k$ represent the leaves in $F'(a)$ (with $k \ge \frac{n}{3}$). Let $Y_1, Y_2,..Y_k$ represent the random variables that query $Q(x_i,b_1,b_2)$ returns $(x,b_1)$ as the closest pair. %Observe that $d(x_i,b_1) = d(x_j,b_1) = d_1$ and $d(x_i,l) = d(x_j,l) =d_2$ for all $i,j \in [k]$.
Let us set $d_1 := d(b_1,b_2)$ and $d_2 := d(x,b_1) = d(x,b_2)$ for any $x \in F'(a)$.
These $\{Y_i\}$s are i.i.d. random variables, each with mean $\frac{d_1+d_2}{2(2d_2 + d_1)}$ - let $\{y_i\}$s be their realizations. Let $Z_1,Z_2,..Z_k$ represent the random variables that query $Q(x_i,b_1,b_2)$ returns $(x_i,l)$ as the closest pair. These $\{Z_i\}$s are i.i.d. random variables, each with mean $\frac{d_1 + d_2}{2(2d_2 + d_1)}$, let $\{z_i\}$s be their realizations. Let $Y = \sum_{i=1}^k y_i$ and $Z = \sum_{i=1}^k z_i$. Observe that $\E[Y] = \E[Z] =: E$, since each of the variables $y_i$ and $z_i$ have identical expectation.


%\\\\
\begin{claim}
With probability at least $1 - \frac{1}{n^6}$, $ |Y-E| < \kappa/2 \sqrt{n \log n}$ and $|Z-E| < \kappa/2 \sqrt{n \log n}$.
\end{claim}

\begin{proof}
%et $T$ be the midpoint between $\E[Y]$ and $\E[Z] + \kappa \fs$. For sufficiently large constant $\tau$ \esh{add specific value}, by the Chernoff bound, we know that the events $Y > T$ and $Z + \kappa \fs < T$ happen with probability at least $1 - \frac{1}{2n^6}$ respectively. An application of the union bound gives that result that $Y > T > Z$ with the desired probability lower bound.

We can see that each inequality happens with high probability, using the Chernoff bound to lower bound the probability of deviations of the sum of $k$ ($\ge \frac{n}{3}$) independent random variables from the mean. Using the union bound over the non-occurrence of the either event gives the desired result.
\end{proof}

Thus, using the triangle inequality, with high probability, we know that $|Y-Z| \le \kappa \sqrt{n \log n}$, ensuring that there is no winner.

\end{proof}




There are two cases to analyze, for each meta-leaf $a$ with $|F'(a)| \ge \frac{n}{3}$. Recall that $T^*$ is the $\sst$ which is rooted at the other child of the parent of the vertex ($v$) at which the $\sst$ corresponding to $F'(a)$ is rooted.

\begin{itemize}
    \item {\bf Case 1 :} There exists a meta-leaf $b \in ML(T') - \{a\}$ such that $F'(b)$ is equivalent to $T^*$ . This case is represented by Figure~\ref{fig:invariants_case1}.
    
    \begin{figure}[h]
        \centering
        \includegraphics[width=10cm]{images/lemma invariants/invariantscase1.png}
        \caption{Case 1: Proof of Correctness of Algorithm~\ref{algorithm:large_familie}}
        \label{fig:invariants_case1}
    \end{figure}
    
    In this case, we claim that the algorithm correctly connects $F'(a)$ and $F'(b)$. Note that any meta-leaf $l \notin ML(T') -\{a,b\}$ will not be present in the sub-tree rooted at vertex $v$. Using Claim~\ref{claim:large_winner}, along with the union bound, the meta-leaf $b$ wins over all $l \notin ML(T') -\{a,b\}$, and is a unique sink in the corresponding tournament graph. Thus, the algorithm connects $F'(a)$ and $F'(b)$, maintaining the invariants. In fact, we prove something stronger, whenever a leaf $a$ witb $|F'(a)| \ge \frac{n}{3}$ has such an adjacent tree $F'(b)$ in the forest we are maintaining, we have shown that, with high probability, $F'(a)$ and $F'(b)$ are always connected  by the first phase of the round algorithm (Algorithm~\ref{algorithm:large_familie}). This is an important property that will be used to argue the overall correctness of our algorithm.
    
    \item{\bf Case 2:} There does not exist a meta-leaf $b \in ML(T') - \{a\}$ such that $F'(b)$ is equivalent to $T^*$. Consequently, there are are at least two meta-leaves $b_1,b_2 \in ML(T') - \{a\}$ such that $F'(b_1)$ and $F'(b_2)$ are equivalent to disjoint $\sst$s of $T^*$. This case is represented by Figure~\ref{fig:invariants_case2}. 
    
    
       
    \begin{figure}[h]
        \centering
        \includegraphics[width=10cm]{images/lemma invariants/invariantscase2.png}
        \caption{Case 2: Proof of Correctness of Algoroithm~\ref{algorithm:large_familie}}
        \label{fig:invariants_case2}
    \end{figure}
    
    
    %Consider any such pair of meta-leaves $b_1$ and $b_2$
    We claim that both $b_1$ and $b_2$ will be sinks in the tournament graph for $a$. Using similar arguments as before (i.e.Claim~\ref{claim:large_winner}), we can see that $b_1$ and $b_2$ win over all meta-leaves $l \notin ML(T') -\{a\}$ not present in the tree rooted at $v$. Additionally, by Claim~\ref{claim:no_winner}, there is no winner in contests between either of $b_1$ and $b_2$ and a meta-leaf $l \notin ML(T') -\{a\}$ that is present in the tree rooted at $v$. Extending this argument for all relevant pairings of meta-leaves (at most $n^2$), and using the union bound, with high probability, there is no unique sink in the tournament graph, and no connection is made by the algorithm, (trivially) preserving the invariants.
    
    
  \end{itemize}    


\subsubsection{Correctness of Algorithm~\ref{algorithm:round_algorithm}}

We need to prove that the second part of Algorithm~\ref{algorithm:round_algorithm} preserves the invariants. The algorithm considers all meta-leaf pairs $a,b$ such that $|F'(a)|,|F'(b)| \le \frac{n}{3}$ and selects one pair that maximizes a certain score. For each pair, this score $s_{a,b}$ is computed as the average number of $(a,b,x)$ queries that return $(a,b)$ for all $x \in L(T) - (F'(a) \cup F'(b))$. We will show that the winning pair $(a,b)$ satisfies the condition that there is no meta-leaf $c \in ML(T')$ such that $(a,b)$ is not the closest pair in the triple $(a,b,c)$. We say that any pair of trees $F'(a), F'(b)$ satisfying these properties are ``sibling trees''. Assuming this to be true, we will show that connecting $a$ and $b$ maintains the invariants. Let $v$ be the root of $F'(a)$, and let $v'$ be the parent of the corresponding $\sst$ in the underlying tree $T$. Then, we argue the $\sst$ corresponding to $F'(b)$ is rooted at the other child, $u$, of $v'$. Assume otherwise, for the sake of contradiction - there are two possibilities. In the first case, $F'(b)$ might be a $\sst$ rooted at an internal, non-root vertex of the $\sst$ rooted at $u$. Consequently, there is at least one other meta-leaf $c$ with $F'(c)$ being the $\sst$ rooted at some other internal vertex (since $F'(b)$, by assumption does not contain all leaves in the tree rooted at $u$). This violates our assumption about $(a,b)$ being the closest pair in all triples of meta-leaves $(a,b,c)$, giving a contradiction. In the other case, $F'(b)$ is the $\sst$ rooted at some internal vertex of the tree $T$ not present in the tree rooted at $v'$. The same argument can be used as in the previous case to reach a contradiction. Thus, the proof is complete if we can prove the stated property about the winning pair $(a,b)$.

Assume, for sake of contradiction, that there exists a meta-leaf $c$ that violates the stated property about the winning pair $(a,b)$. Without loss of generality, let $(b,c)$ be the closest pair of the triple $(a,b,c)$. 
%Let $e$ be a meta-leaf that minimizes the distance $d(c,e')$ over all $d' \in ML(T') - \{c\}$. Note that $e$ may not be unique, however any such $e$ works for the sake of this proof. 
Consider the subtree rooted at the least common ancestor of $b$ and $c$. We claim that there is at least one pair of ``sibling'' trees $F'(e)$ and $F'(f)$ within this subtree ($e,f \in ML(T')$,i.e., trees such that there exists no other meta-leaf $g$ where $(e,f)$ is not the smallest pair in $(e,f,g)$. %Additionally, we will show that there exists such a pair $e,f$ in the subtree containing $F'(b)$ rooted at the least common ancestor of $a$ and $b$. 
This is demonstrated via a constructive proof. For any $l \in ML(T')$, let $CL(l)$ represent the meta-leaves $l'$ in $ML(T')\setminus \{l\}$ that minimize the distance $d(l,l')$.  Notice that it suffices to prove that there exists $e,f \in ML(T')$ such that $e \in CL(f)$ and $f \in CL(e)$. Implicitly, these sets will be singleton, through the property that every triple of leaves has a unique closest pair. Start with $c' = c$. %We know that $a \notin CL(b)$. 
Consider $c''$, which is some leaf in $CL(c')$. If $c' \in CL(c'')$, we have our desired pair $(c',c'')$. Otherwise, set $c' = c''$ and repeat the process. Our algorithm can always proceed, since $CL(l)$ is non-empty for any meta-leaf $l \in ML(T')$. Additionally, our algorithm will always terminate since the quantity $d(c',c'')$ strictly decreases in each step. Finally, observe that, when the algorithm terminates, we have that $|F'(c)|,|F'(c'')| < \frac{n}{3}$. Assume otherwise - then we know that the algorithm to connect large families would have connected them before reaching this step, leading to a contradiction.

We will show that, with high probability, $(e,f)$ has a better score than $(a,b)$, thus contradicting the status of $(a,b)$ as the highest scoring pair.
 
 \begin{claim}
 With high probability, $(e,f)$ has a better score than $(a,b)$.
 \end{claim}
\esh{Need to add this proof - one unresolved case}

We have shown that the algorithm preserves the desired invariants with each step, and that when the algorithm terminates, it terminates with the correct answer. The final step left to prove is that the algorithm makes progress in every round, i.e., to prove Lemma~\ref{lemma:progress}.

At the beginning of each round (before completion, there are at least two vertices), we first observe that there is some pair of vertices $a,b \in ML(T')$ such that $a \in CL(b)$ and $b \in CL(a)$ (we have already shown a constructive proof of existence). Implicitly, $CL(a)$ and $CL(b)$ are singleton sets. First, consider the case where either of $|F'(a)|$ or $|F'(b)|$ is greater than or equal to $\frac{n}{3}$. We have already seen that Algorithm~\ref{algorithm:large_familie} (the subroutine that acts on large families) will connect $a$ and $b$ in this case, ensuring progress. Otherwise, we have $|F'(a)|, |F'(b)| \le \frac{n}{3}$. Since there is at least one such pair fulfulling this condition, the second part of Algorithm~\ref{algorithm:round_algorithm} necessarily connects some pair of meta-leaves, ensuring progress and completing the proof of Lemma~\ref{lemma:progress}.
 
    
%\end{itemize}







==> old content/old_notation.tex <==
The most general binary trees that we can consider in the context of evolution are full binary trees, which are binary trees in which every internal node has exactly two children (corresponding to a species evolving into two distinct species). We will give an algorithm that exactly reconstructs any binary tree under the condition that the length of each edge is at least $\tau \fs$. For convenience, the height of the tree $h(T)$ is henceforth normalized to be $1$.

%Our first step is to define $i$-th cousins to ensure that the relation is symmetric. 
\begin{definition}
The unweighted height of a vertex $v$, $UHT(v)$ is defined as the the largest index $i \in \{0,1,2\cdots,n\}$ such that $v$ has an $i$-th descendant in the tree but does not have a $j$-th descendant for any $j > i $.
\end{definition}
We can alternatively think of a recursive definition for unweighted height - every leaf has unweighted height $0$ and the unweighted height of an internal node is defined as one plus the larger of the unweighted heights of its children. Importantly, observe that this relation is symmetric.


\begin{definition}
Two leaf nodes $a$ and $a'$ are $i$-th cousins of each other if their least common ancestor has unweighted height $i+1$. 
\end{definition}

Thus, siblings leaves are $0-th$ cousins, and for convenience, each leaf can be thought of as its own $(-1)-th$ cousin.

Let $C_i(a)$ represent the set of $i$th cousins of leaf $a$. Set $C_{-1}(a)= a$ for all leaves $a$. Let $F_k(a) = \cup_{i = -1}^k C_i(a)$. Note that $F_k(a)$ is the set of leaves in the sub-tree rooted at the $k+1$-th ancestor of $a$.

%The sets $C_i(a)$ and $F_{i-1}(a)$ have the same meaning as the previous section. 
Note that with this definition, the $i$-th cousin relation is symmetric i.e., $a \in C_i(a') \implies a' \in C_i(a)$. This definition immediately leads us to a useful lemma about any two leaves that are $i$-th cousins of each other.

\begin{lemma}
\label{lemma:cousin_constraints}
Let $a$ and $a'$ be $i$-th cousins of each other, with $i > 0$. Then, at least one of these vertices has an $i-1$-th cousin.
\end{lemma}
\begin{proof}
Let $p$  be the least common ancestor of $a$ and $a'$. Observe that $a$ and $a'$ are contained in different sub-trees of $p$. We know that the unweighted height of $p$ is $i+1$. Using the recursive definition of unweighted height, we know that at least one of $p$'s children has unweighted height $i$. Let this child be $q$, WLOG, let $a$ be contained in the sub-tree rooted at $q$. Note that $i > 0$, which implies that $q$ is an internal node of the tree and thus has two sub-trees, both of which contain at least one leaf. Thus, the leaf $a$ has at least one $i-1$-th cousin.
\end{proof}

\esh{This paragraph might have to be moved up to the model}
In context of our problem, we do not care about the labels for internal vertices of a tree. In comparing two trees for similarity, we only care about the labels on the leaves and their relative arrangements. In particular, consider a relabeling of any given rooted tree - where all internal vertices are labelled in terms of the leaves. To give a recursive definition, each leaf $l$ is its own label $Lab(l) = l$. The label of any internal vertex $v$ is $Lab(v) : = Lab(lc) + Lab(rc)$ where $lc$ and $rc$ are its left and right child respectively, and $+$ represents the append operation. Two full binary trees (given along with a root) are equivalent in our model if:
\begin{enumerate}
    \item They have the same set of leaf labels.
    \item After relabelling the internal vertices based on the leaves, they are the exact same tree.
\end{enumerate}

\esh{Need to mention in the model that the underlying tree is structured in a very particular way, rooted at the common ancestor of all species and having the children relation correspond to an ``immediate'' evolution of the parent species.}

As a consequence of this definition of equivalence, we have the following lemma.

\begin{lemma}
Two trees $T_1$ and $T_2$ are equivalent in our model, if they have the same leaf sets, i.e., $L(T_1) = L(T_2)$ and the cousin relations $C_{T_1}$ and $C_{T_2}$ are the same function.
\end{lemma}

\begin{definition}
A $\sst$ t \esh{Better name? We can swap out the macro accordinglt} of the tree $T$ is the subtree rooted at some vertex $v$ of $T$. Note that every $\sst$ t is also a full binary tree.
\end{definition}


Unlike perfect binary trees, full binary trees do not guarantee the existence of an $i$-th cousin for any leaf $a$. In fact, it is possible that some leaf $a$ has an arbitrary set of cousins in $\{0,1,2\cdots n\}$. However, the above lemma tells us that there is some structure when we look at the cousin sets of all leaves in the tree.

==> old content/old_proofs_full_trees.tex <==
























\begin{comment}
\subsection{Proof of Lemma~\ref{lemma:behave_alike}}

Consider the first part of the lemma. $a$ and $b$ are correctly in the $i$-th round, with $i<t$. Consider the test $O^t_c(b,d)$ with $c,d \notin F_{t-1}(a)$. If this test returns a result, then it must have fallen into either regime 1 $|F^{t-1}_{t-1}(b)| \ge \frac{2n}{9}$ or regime 2. In either regime, note that every leaf $x$ used to compare $b$ and $d$ comes from outside $F^{t-1}_{t-1}(b)$ and hence, from outside $F_{t-1}(b)$ since the inductive assumption on the invariants assure us that $F_{t-1}(b) \subseteq F^{t-1}_{t-1}(b)$.
\end{comment}


==> old content/perfect_trees.tex <==
In this section, we work on reconstructing the perfect binary tree with $n$ leaves, armed with the condition that the length of each edge is $\Omega\left(\frac{h(T) \log n}{\sqrt{n}} \right)$.

To aid the description of the algorithm, we define the $k$-th cousin of any leaf vertex $a$. Consider the $k+1$-th ancestor of leaf $a$, call this vertex $v$, and let $v'$ be the $k$-th ancestor of $a$. Let $v''$ be the  other child of $v$ (that is not $v'$). Let $T(u)$ denote the sub-tree rooted at any vertex $u$. All leaves in the sub-tree $T(v'')$ are called the $k$-th cousins of the leaf $a$. Observe that the $0$-cousin of a leaf is its sibling. Also note that, in the case of perfect binary trees, $i$-th cousinhood is a symmetric relation. \esh{Will be changing this definition for general trees to preserve this property}

Since we are working with a perfect binary tree, i.e., a tree where all internal nodes have two children and all leaves are at the same depth, we know that every leaf $a$ has an $i$th sibling, for $i=0$ to $i=\log n$ (which is an integer by our assumption). %To generalize the results of this section to all binary trees, we will need to 

Let $C_i(a)$ represent the set of $i$th cousins of leaf $a$. Set $C_{-1}(a)= a$ for all leaves $a$. Let $F_k(a) = \cup_{i = 0}^k C_i(a)$. Note that $F_k(a)$ is the set of leaves in the sub-tree rooted at the $k+1$-th ancestor of $a$ (with leaf $a$ exempted).

The algorithm proceeds in rounds, where, in the $i$-th round (starting from $i=0$), we find the $i$-th cousin set $C_i(a)$ for every leaf $a$. Alternatively, the algorithm can be thought of as constructing the forest generated by the bottom $i+1$ levels of the tree in round $i$. Observe that we will have reconstructed the entire tree after finding $C_i(a)$ for all leaves $a$ from $i=0$ to $\log n$. We will look at the base case of $i=0$ and then show how to construct $C_i(a)$ given $F_{i-1}(a)$ for all leaves $a$.

This may not be the most efficient algorithm, either in terms of time or more importantly, the number of queries made to the oracle $Q$.\esh{Will come back to this question after generalizing the algorithm for all binary trees}
\subsection{Finding the Sibling of Every Leaf}
For $i=0$, we are finding the sibling of each leaf $a$. Let $a'$ be the sibling leaf of $a$ (which is, of course, not known to us beforehand). This leaf $a'$ displays a useful property that can be used to identify it uniquely. Consider the following test that takes as input two arbitrary leaves $b,c$ and compares $d(a,b)$ and $d(a,c)$, returning the closer leaf. To help with notation, we represent this test as an algorithm $O^0_a$ that takes two leaves $b,c$ as input and returns one of them. 


Let $S$ be the set of all leaves $x$ that are not $a,b$ or $c$, i.e., $S = L(T) - \{a,b,c\}$. Iterate over all leaves $x \in S$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $h_x$ and $w_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ (respectively $(a,c)$). Let $H = \sum_x  h_x$ and $W = \sum_x w_x$. If $H \ge W + \alpha \sqrt{n} \log n$, the test returns $b$, i.e., $O^0_a(b,c) = b$, else if $W \ge H + \alpha \sqrt{n} \log n$, $O^0_a(b,c) = c$, if neither criterion is satisfied - the test returns no answer.

The sibling $a'$ of leaf $a$ has the following useful property-

\begin{lemma}
\label{lemma:sibling_ft}
For all leaves $c \in L(T) - \{a,a'\}$, whp, $O^0_a(a',c) = O^0_a(c,a') = a'$. 
\end{lemma}

\begin{proof}
We prove that $O^0_a(a',c)  = a'$, it will be clear that the same proof can be used to show $O^0_a(c,a') = a'$.
We know that $d(a,a')  < d(a,c)$ for all $c \in L(T) - \{a,a'\}$. Let $p$  be the least common ancestor of $a$ and $a'$ (in fact, their first ancestor), and let $q$ be the least common ancestor of $a,a',c$. Let $S = L(T) - \{a,a',c\}$. We will prove the following claim
\begin{claim}
\label{claim:local_sibling_ft}
$\expect{h_x} - \expect{w_x} = \Omega\left(\frac{w_{min}}{h(T)}\right)$ for every leaf $x \in S$.
\end{claim}
 The proof of this claim has been moved to Appendix~\ref{subsection:pf_sibling_ft}. If this is shown to be true, we will have $\expect{H} - \expect{W} = \Omega \left ( \frac{n w_{min}}{h(T)} \right) \ge \kappa \sqrt{n} \log n$. Observe that both $H$ and $W$ are the sum of $n$ independent $0-1$ random variables, the application of the Chernoff bound tell us, that with high probability (greater than $1-\frac{1}{2n^6}$), that $\expect{H} - H \le \frac{\kappa}{3}\sqrt{n} \log n$ and $W - \expect{W} \le \frac{\kappa}{3}\sqrt{n} \log n$. Thus, using the union bound, we will have $H \ge W + \frac{\kappa}{3} \sqrt{n} \log n$ with probability at least $1 - \frac{1}{n^6}$.
\end{proof}

Lemma~\ref{lemma:sibling_ft} gives a natural algorithm to identify the sibling of any leaf vertex $a$. Let $S^0_a = L(T) - \{a\}$. Construct the directed graph $G^0_a$ on vertices $S^0_a$ as follows. Iterate over all pairs of leaves $b,c$ in $S^0_a$, compute $O^0_a(b,c)$. Draw an edge from $b$ to $c$ if $O^0_a(b,c) = c$, otherwise, draw an edge from $c$ to $b$. Observe that the output of $O^0_a$ (the winner of every pair) defines a tournament among the vertices $S^0_a$. Lemma~\ref{lemma:sibling_ft} implies that the graph $G^0_a$ has a unique sink, which is in fact the sibling of $a$.

\subsection{Finding the $i$-th Cousin of Every Leaf}
Moving on to the problem of finding the $i$-th cousin of vertex $a$, given that we know $F_{i-1}(x)$ for all leaves $x$. Note that it suffices to find even a single vertex $a' \in C_i(a)$, 
since all the other vertices in $C_i(a$0 will be the $j$-th cousins of leaf $a'$ for some $j \in \{0,1,2,...i-1\}$.i.e., $C_i(a) = \{a'\} \cup F_{i-1}(a')$. Let $S^i_a = L(T) - \{a\} - F_{i-1}(a)$, i.e., $S^i_a$ is the set of candidate leaves for $i$-th cousins of leaf $a$. Consider the following test, $O^i_a$, that takes as input two leaves $b,c$ in $S^i_a$ and compares $d(a,b)$ versus $d(a,c)$.



Set $S = S^i_a - \{b,c\} -  F_{i-1}(b) -F_{i-1}(c)$. The test can take place in one of two regimes -either if $|F_{i-1}(a)| \ge \frac{2n}{9}$ is true or if $|S| \ge \frac{n}{3}$ is true. If neither condition is satisfied, the test fails to return an answer.  %\esh{The second regime is not needed for the full binary trees case, however it will be useful for thinking about generic binary trees}

For the first regime, where $|F_{i-1}(a)| \ge \frac{2n}{9}$- iterate over all $x \in F_{i-1}(a) \cup \{a\}$ and record the results of the query $(x,b,c)$. Let $f_x$ and $g_x$ be the indicator variables that are set to $1$ when $Q(x,b,c)$  returns $(x,b)$ (respectively $(x,c)$). Let $F = \sum_x  f_x$ and $G = \sum_x g_x$. If $F \ge G + \alpha \sqrt{n} \log n$, the test returns $b$, i.e., $O^0_a(b,c) = b$, else if $G \ge F + \alpha \sqrt{n} \log n$, $O^0_a(b,c) = c$, if neither criterion is satisfied - the test returns no answer.

For the second regime, where $|S| \ge \frac{n}{3}$ - Iterate over all leaves $x \in S$ and record the results of the queries $(a,c,x)$ and $(a,b,x)$. Let $h_x$ and $w_x$ be the indicator variables that are set to $1$ when $Q(a,b,x)$ (respectively $Q(a,c,x)$) returns $(a,b)$ (respectively $(a,c)$). Let $H = \sum_x  h_x$ and $W = \sum_x w_x$. If $H \ge W + \alpha \sqrt{n} \log n$, the test returns $b$, i.e., $O^0_a(b,c) = b$, else if $W \ge H + \alpha \sqrt{n} \log n$, $O^0_a(b,c) = c$, if neither criterion is satisfied - the test returns no answer.

\begin{lemma}
\label{lemma:cousin_ft_reg1}
Let leaf $a$ satisfy the property that $|F_{i-1}(a)| \ge \frac{2n}{9}$. Let $a'$ be an $i$-th cousin of $a$, then, whp, $O^i_a(a',c) = O^i_a(c,a') = a'$ for all $c \in S^i_a - C_i(a)$ ,i.e., under the right conditions, an $i$-th cousin of leaf $a$ almost always wins over a more distant cousin of $a$ in the test $O^i_a$.
\end{lemma}

\begin{proof}
We prove that $O^0_a(a',c)  = a'$, it will be clear that the same proof can be used to show $O^0_a(c,a') = a'$.
We know that $d(a,a')  < d(a,c)$ for all $c \in S^i_a - C_i(a)$. Let $p$ be the least common ancestor of $a$ and $a'$ (in fact, their $i+1$-th ancestor), and let $q$ be the least common ancestor of $a,a',c$. 

Based on the conditions in the lemma, observe that the test $O^0_a(a',c)$ will fall into the first regime.

 \begin{claim}
 \label{claim:local_cousin_ft_reg1}
 $\expect{f_x} - \expect{g_x} = \Omega\left(\frac{w_{min}}{h(T)}\right)$ for every leaf $x \in F_{i-1}(a) \cup \{a\}$.
 \end{claim}
The proof of this claim has been moved to Appendix~\ref{subsection:local_cousin_ft_reg1}. If this is shown to be true, we will have $\expect{F} - \expect{G} = \Omega \left ( \frac{n w_{min}}{h(T)} \right) \ge \kappa \sqrt{n} \log n$. Observe that both $F$ and $G$ are the sum of $n$ independent $0-1$ random variables, the application of the Chernoff bound tell us, that with high probability (greater than $1-\frac{1}{2n^6}$), that $\expect{F} - F \le \frac{\kappa}{2}\sqrt{n} \log n$ and $G - \expect{G} \le \frac{\kappa}{2}\sqrt{n} \log n$. Thus, using the union bound, we will have $F \ge G$ with probability at least $1 - \frac{1}{n^6}$.
\end{proof}

\begin{lemma}
\label{lemma:cousin_ft_reg2}
Let leaf $a$ satisfy the property that $|F_{i-1}(a)| < \frac{2n}{9}$. Let $a'$ be an $i$-th cousin of $a$, and let leaf $c \in S^i_a - C_i(a)$ satisfy the conditions that $|F_{i-1}(a')|, |F_{i-1}(a')| < \frac{2n}{9}$, then, whp, $O^i_a(a',c) = O^i_a(c,a') = a', $i.e., under the right conditions, an $i$-th cousin of leaf $a$ almost always wins over a more distant cousin of $a$ in the test $O^i_a$.
\end{lemma}

\begin{proof}
We prove that $O^0_a(a',c)  = a'$, it will be clear that the same proof can be used to show $O^0_a(c,a') = a'$.
We know that $d(a,a')  < d(a,c)$ for all $c \in S^i_a - C_i(a)$. Let $p$ be the least common ancestor of $a$ and $a'$ (in fact, their $i+1$-th ancestor), and let $q$ be the least common ancestor of $a,a',c$. 


 Recall that $S = S^i_a - \{a',c\} -  F_{i-1}(a') -F_{i-1}(c)$. Using the conditions in the lemma, $|S| \ge \frac{n}{3}$. Thus, the test $O^0_a(a',c)$ will fall into the second regime.
\begin{claim}
\label{claim:local_cousin_ft_reg2}
$\expect{h_x} - \expect{w_x} = \Omega\left(\frac{w_{min}}{h(T)}\right)$ for every leaf $x \in S$.
\end{claim}
 This correctness of this claim can be argued using arguments similar to those used to prove Claim~\ref{claim:local_sibling_ft} (found in Appendix~\ref{subsection:pf_sibling_ft}). This is because, the only assumption that the proof in Appendix~\ref{subsection:pf_sibling_ft} makes is that $x \notin L(T(p))$ (recall that $p$ is the least common ancestor of $a$ and $a'$). Observe that $p$ is the $i+1$-th ancestor of both $a$ and $a'$, and that they are in different sub-trees of $p$, since $p$ is the least common ancestor. Thus, $L(T(p)) = \{a\} \cup F_{i-1}(a) \cup \{a'\} \cup F_{i-1}(a')$. By definition of $S$, we have $S \cap L(T(p)) = \phi$, thus $x \notin L(T(p))$.
 
 With the above claim, we will have $\expect{H} - \expect{W} = \Omega \left ( \frac{n w_{min}}{h(T)} \right) \ge \kappa \sqrt{n} \log n$. Observe that both $H$ and $W$ are the sum of $n$ independent $0-1$ random variables, the application of the Chernoff bound tell us, that with high probability (greater than $1-\frac{1}{2n^6}$), that $\expect{H} - H \le \frac{\kappa}{3}\sqrt{n} \log n$ and $W - \expect{W} \le \frac{\kappa}{3}\sqrt{n} \log n$. Thus, using the union bound, we will have $H \ge W + \frac{\kappa}{3}\sqrt{n}$ with probability at least $1 - \frac{1}{n^6}$.
\end{proof}


The algorithm to find the $i$-th cousin of all vertices proceeds in two phases. In the first phase, the algorithm finds the set of $i$-th cousins of all leaves $a$ with $|F_i(a)| \ge \frac{2n}{9}$, by utilizing the first regime of the test $O^i_a$. Note that, since the $i$-th cousin relationship is symmetric in perfect binary trees, the algorithm might also find the set of $i$-th cousins of leaves $a$ not satisfying $|F_i(a)| \ge \frac{2n}{9}$.

In the second phase, the algorithm finds the $i$-th cousins of the ``leftover'' leaves, i.e., leaves $a$ such that $|F_{i-1}(a)| < \frac{2n}{9}$ and for all $x \in C_i(a)$, $|F_{i-1}(x)| \le \frac{2n}{9}$. This phase of the algorithm utilizes the second regime of the test $O^i_a$.

The algorithm is described in full detail as Algorithm~\ref{algorithm:cousins}.

{	
\begin{algorithm}[ht]
	{
		\label{algorithm:cousins}
			\caption{Algorithm for Finding $i$-th cousins of all Leaves}
		\begin{algorithmic}[1]
		%\STATE x=5
		\STATE Set $\X = L(T)$.
		\STATE \COMMENT{Phase 1 of the Algorithm:}
		\WHILE{$\exists a \in \X$ such that $|F_i(a)| \ge \frac{2n}{9}$} 
        \FOR{$b,c \in S^i_a$}                    
        \STATE  In the graph $G^i_a$, draw an edge from $b$ to $c$ if $O^0_a(b,c) = c$ and $c \notin F_{i-1}(b)$, alternatively, draw an edge from $c$ to $b$ if $O^0_a(b,c) = b$ and $b \notin F_{i-1}(c)$
        \ENDFOR
        \STATE Let $a'$ be a sink of $G^i_a$
        \FOR{$a^* \in F_{i-1}(a) \cup \{a\}$}
        \STATE Set $C_i(a^*) = \{a'\} \cup F_{i-1}(a')$
        \ENDFOR
        \FOR{$a'' \in F_{i-1}(a') \cup \{a'\}$}
        \STATE Set $C_i(a'') = \{a\} \cup F_{i-1}(a)$
        \ENDFOR
        \STATE Update $\X \leftarrow \X - (\{a \} \cup \{a'\} \cup F_{i-1}(a)- \cup F_{i-1}(a'))$
      \ENDWHILE\label{while:phase1}
      \STATE Record $\X_1 = L(T) - \X$, $\X_2 = \X$
      \STATE \COMMENT{Phase 2 of the Algorithm:}
    \WHILE{$\exists a \in \X$} 
        \FOR{$b,c \in S^i_a$ such that $|F_{i-1}(b)|,|F_{i-1}(c)| < \frac{2n}{9}$} %\esh{Equivalently, $b,c \in \X_2$}      
        \STATE  In the graph $G^i_a$, draw an edge from $b$ to $c$ if $O^0_a(b,c) = c$ and $c \notin F_{i-1}(b)$, alternatively, draw an edge from $c$ to $b$ if $O^0_a(b,c) = b$ and $b \notin F_{i-1}(c)$.
        \ENDFOR
        \STATE Let $a'$ be a sink of $G^i_a$
        \FOR{$a^* \in F_{i-1}(a) \cup \{a\}$}
        \STATE Set $C_i(a^*) = \{a'\} \cup F_{i-1}(a')$
        \ENDFOR
        \FOR{$a'' \in F_{i-1}(a') \cup \{a'\}$}
        \STATE Set $C_i(a'') = \{a\} \cup F_{i-1}(a)$
        \ENDFOR
        \STATE Update $\X \leftarrow \X - (\{a \} \cup \{a'\} \cup F_{i-1}(a)- \cup F_{i-1}(a'))$
      \ENDWHILE\label{while:phase1}
      
		\end{algorithmic}
    }
	\end{algorithm}
}		

%Lemma~\ref{lemma:cousin_ft} gives a natural algorithm to identify an $i$-th cousin of any leaf vertex $a$. Construct the directed graph $G^i_a$ on vertices $S^i_a$ as follows. Iterate over all pairs of leaves $b,c$ in $S^i_a$, compute $O^0_a(b,c)$. Draw an edge from $b$ to $c$ if $O^0_a(b,c) = c$ and $c \notin F_{i-1}(b)$, alternatively, draw an edge from $c$ to $b$ if $O^0_a(b,c) = b$ and $b \notin F_{i-1}(c)$. 

Analyzing the first phase, for each leaf $a$ considered  (i.e., with $F_{i-1}(a)| \ge \frac{2n}{9}$, Lemma~\ref{lemma:cousin_ft_reg1} implies that the set of sinks of $G^i_a$ is exactly the set of $i$-th cousins of $a$. 

For the forward direction, consider any sink $x$ of $G^i_a$. Assume $x \notin C_i(a)$. Consider some leaf $a'$ that is an $i$-th cousin of $a$. Note that, for a perfect binary tree, such a leaf always exists. \esh{this is the assumption we will have to get around for general binary trees}. We know that $a' \notin F_{i-1}(x)$ since that would imply that $x$ is also an $i$-th cousin of $a$. Additionally, by Lemma~\ref{lemma:cousin_ft_reg1}, $O^i_a(a',x) = a'$. Thus, there will be an edge from $x$ to $a'$, contradicting the assumption that $x$ was a sink.

For the reverse direction, consider any $a' \in C_i(a)$. Assume $a'$ is not a sink, i.e., there is an edge $(a',x)$ in the graph $G^i_a$. We know that if $x \notin C_i(a)$, then $O^i_a(a',x) = a'$, ruling out the possibility of edge $(a',x)$. Thus, we are forced to have $x \in C_i(a)$, this would imply that $x \in F_{i-1}(a')$, again ruling out the the possibility of edge $(a',x)$. Thus, we have a contradiction.

Consequently, any sink of $G^i_a$ will be an $i$-th cousin of the leaf $a$, and the existence of a sink is guaranteed by the existence of an $i$-th cousin for leaf $a$ (since we are dealing with perfect binary trees).


 Observe that if a leaf $a$ is present in the set of leftover leaves $\X_2$ after the first phase, then we have $|F_{i-1}(a)| < \frac{2n}{9}$ and for all $x \in C_i(a)$, $|F_{i-1}(x)| \le \frac{2n}{9}$. Thus, similar arguments can be used to show that the $i$-th cousin of all remaining leaves is correctly found by the algorithm, by employing Lemma~\ref{lemma:cousin_ft_reg2} instead of Lemma~\ref{lemma:cousin_ft_reg1}, since the second regime of testing is active for all tests of the form $O^i_a(a',c)$, where $a'$ is an $i$-th cousin of $a$ and $c$ is a $j$-th cousin of $a$ with $j > i$, made by the algorithm.

This completes the algorithmic reconstruction of perfect binary trees.

\subsection{A Note about Robustness}

Since our tests are based on comparing sums of random variables, we can add in some noise to our query model without losing out on the results above. In particular, we can come up with bounds on how much Gaussian/adversarial noise to the queries without losing the results above. \esh{Is this worth pursuing?} \esh{Alternatively, we can also explore whether minor deviations from the ultrametric property are smoothed out by our algorithm.}
%since all the $j$-th cousins of $a'$, for $j=0$ to $i-1$ of $a'$ will also be the $i$-th cousins of leaf $a$. In fact, every $i$-th cousin of $a$ will be present in the set $F_{i-1}(a') \cup \{a'\}$.




==> proofs/build_trees.tex <==
%$T_S$ is the induced tree on $S$. 
We build subtrees of $T_S$ from the ground up, starting with each leaf in $S$ as a singleton subtree. Let $T_1, T_2, \cdots T_l$ represent subtrees of $T_S$ whose leaves form a disjoint partition of $S$ - we show an algorithm, that with high probability, combines two of these subtrees to form a larger subtree of $T_S$. Let $L_i$ represent the set of leaves of $T_i$. Using this procedure, we start with the initial configuration and repeatedly keep applying this step until the size of the largest subtree exceeds $\sqrt{n} - 1$. Since each step can at most double the size of the largest subtree, we obtain a subtree of $T_S$ of size in the range $[\sqrt{n}, 2 \sqrt{n}]$.

Now, we describe the algorithm.
For each pair $T_i, T_j$, we generate a score $s_{ij}$ in the following manner. Fix arbitrary $a \in L_i$, and $b \in L_j$.  Define a $0-1$ random variable $X^x_{ij}$ for each leaf $x \in S \setminus (L_i \cup L_j)$ to be $1$ if the query $Q(a,b,x)$ gives $(a,b)$ as the answer, and 0 otherwise.
\[s_{ij} = \frac{\sum_{x \in S \setminus (L_i \cup L_j
)} X^x_{ij}}{| S \setminus (L_i \cup L_j
)|} \]
We claim that (whp) the tree pair with the highest score is in fact a ``sibling - tree pair'', i.e., a pair of subtrees of $T_S$ that can be combined through a shared parent internal node to form a subtree of $T_S$. There always exists such a sibling-tree pair, since these leaf-disjoint subtrees of $T_S$ themselves form a full binary tree. 

\hide{
We start with a simple observation: For any pair $T_k, T_l$ that is not a sibling pair, there is a sibling pair
$T_i, T_j$ such that the distance between arbitrary representative leaves $a \in L_i$ and $b \in L_j$ is less than the distance between arbitrary leaves $c \in L_k$ and $d \in L_l$.
}

We start with a simple observation: For any pair $T_k, T_l$ that is not a sibling pair, there is a sibling pair
$T_i, T_j$ such that their least common ancestor is strictly below the root of either $T_k$ or $T_l$.


To see this we consider the full binary tree resulting from starting with $T$ and collapsing each set of leaves $L_i$ into a single node and look at the subtree rooted at the least common ancestor of $T_k$ and $T_l$. There must be a deepest internal node in this tree whose children are sibling subtrees $T_i$ and $T_j$, completing the proof. Figure~\ref{fig:score_winner} shows such a set of trees.

 %Clearly the distance between $T_i$ and $T_j$ is less than the distance between $T_k$ and $T_l$.

\begin{figure}
    \centering
    \includegraphics[width=6cm]{new_images/score_winner_updated.png}
    \caption{Sibling-Tree Pair between Non Sibling-Tree Pair}
    \label{fig:score_winner}
\end{figure}


\hide{
 $T_a, T_b$, then there exists a sibling-tree pair $T_c, T_d$ such that either $d(T_a, T_c) < d(T_a,T_b)$ or $d(T_b, T_c) < d(T_a,T_b)$ (Ref Fig~\ref{fig:score_winner}). %the $LCA_{T_S}(T_b,T_c,T_d)$ is below $LCA_{T_S}(T_a,T_b)$ within $T_S$ or the $LCA_{T_S}(T_a,T_c,T_d)$ is below $LCA_{T_S}(T_a,T_b)$ within $T_S$. Here $LCA_{T_S}$ represents the least common ancestor relation within the induced tree $T_S$. 
\begin{figure}
    \centering
    \includegraphics[width=6cm]{new_images/score_winner.png}
    \caption{Sibling-Tree Pair between Non Sibling-Tree Pair}
    \label{fig:score_winner}
\end{figure}
For proof -%, since $T_a, T_b$ is a non sibling-tree pair. 
Set $e = a, f = b$. If $T_e$ and $T_f$ are a sibling-tree pair, then we are done. Otherwise, there exists (WLOG), an index $g$ exists such that $d(T_e, T_g) < d(T_e,T_f)$ - in which case we set $f=g$ and continue. In each step, we strictly reduce $d(T_e, T_f)$ and hence eventually reach the desired condition.
}

\begin{claim}
With high probability, $s_{kl} < s_{ij}$.
\end{claim}
\sk{The notation in this claim is inappropriate.. You used $i,j,$ etc. to index subtrees and $a, b, $ etc. to index leaves in these subtrees. You defined scores with subscripts $i,j,$, not $a, b$... to be correct here, we need to map $a$ to $k$, $b$ to $l$, $c$ to $i$ and $d$ to $j$. Also, the proof below is unnecessarily complicated and notation-heavy.
Could you not define so many different sets and quantities? Just explain how for all but $O(\sqrt{n})$ leaves we get a strong signal that the noise from the remaining $\sqrt n$
leaves will not dampen the signal..
}


%Hide begins


\hide{
\begin{proof}
Let $S_1 : = S \setminus (L_k \cup L_l)$ and $S_2 : = S \setminus (L_i \cup L_j)$. $S_1$ is the set of leaves used to compute the score $s_{kl}$ and $S_2$ is the set of leaves used to compute the score $s_{ij}$. Since $|L_k|, |L_l|, |L_i|, |L_j| \le 2 \sqrt{n}$, we can assume that $|S_1|, |S_2| \ge \frac{n}{16}$. Define $A := S_1 \cap S_2$, $B_1 := S_1 \setminus S_2$ and $B_2 := S_2 \setminus S_1$. Now $B_1 = L_i \cup L_j$ and $B_2 = L_k \cup L_l$. Thus $z := |A| \ge \frac{n}{16}$ and $q_1 := |B_1|, q_2 := |B_2| \le 4\sqrt{n}$. Using the condition on minimum edge length, it is not hard to see (Ref~Fig~\ref{fig:score_winner}) that :
\[ \forall x \in A: \E[X^x_{ij}]  - \E[X^x_{kl}] \ge \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \]
\[ \forall x \in B_2, y \in B_1: \E[X^x_{ij}]  - \E[X^y_{kl}] \ge \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \]

\esh{Should I include a proof of these two inequalities? Maybe rewrite them as a claim, so that we can push the proof to the appendix?}
\sk{May be not... since they seem pretty easy? Just state and say something like it is not hard to see... unless I am missing something.}
\esh{Done}

We can write $S_1 = A \cup B_1$ and $S_2 = A \cup B_2$. Thus: 
\[s_{kl} = \frac{\sum_{x \in A}X^x_{ab } + \sum_{y \in B_1}X^y_{ab }}{|A| + |B_1|} \]

\[s_{ij} = \frac{\sum_{x \in A}X^x_{cd } + \sum_{x \in B_2}X^x_{cd }}{|A| + |B_2|} \]

% $s_{kl}$ and $s_{ij}$ are also random variables. 
We will compare the random variables $T_1 := |S_1||S_2| s_{kl}$ and $T_2 := |S_1||S_2| s_{ij}$. %If we can show that $T_2 - T_1 > 0$ with high probability, then we are done. 
We know $q_1 := |B_1|, q_2 := |B_2| \le 4\sqrt{n}.

\[ T_1 = z \sum_{x \in A}X^x_{ab } + q_2 \sum_{x \in A}X^x_{ab } + z \sum_{y \in B_1}X^y_{ab } + q_2 \sum_{y \in B_1}X^y_{ab } \]

\[ T_2 = z \sum_{x \in A}X^x_{cd } + q_1 \sum_{x \in A}X^x_{cd } + z \sum_{x \in B_2}X^x_{cd } + q_1 \sum_{x \in B_2}X^x_{ab } \]


{\bf Case 1: $|B_1| \ge |B_2|$ i.e. $q_1 \ge q_2$ :} 
Let $B'_1 \subset B_1$ be any subset such that $|B'_1| = |B_2|$
\begin{align*}
    T_2 - T_1 &= z (\sum_{x \in A}(X^x_{cd } - X^x_{ab })) + (q_1 \sum_{x \in A}X^x_{cd } - q_2 \sum_{x \in A}X^x_{ab }) + z(\sum_{x \in B_2}X^x_{cd } - \sum_{y \in B_1}X^y_{ab }) + (q_1 \sum_{x \in B_2}X^x_{ab } - q_2 \sum_{y \in B_1}X^y_{ab }) \\
    &\ge z (\sum_{x \in A}(X^x_{cd } - X^x_{ab })) + (q_1 \sum_{x \in A}X^x_{cd } - q_1 \sum_{x \in A}X^x_{ab }) + z(\sum_{x \in B_2}X^x_{cd } - \sum_{y \in B'_1}X^y_{ab }) - \sum_{y \in B_1 \setminus B'_1}X^y_{ab } \\
    & \quad + (q_1 \sum_{x \in B_2}X^x_{ab } - q_2 \sum_{y \in B_1}X^y_{ab })
\end{align*}

On the right hand side, %we can make the second term smaller by replacing it by $(q_2 \sum_{x \in A}X^x_{cd } - q_2 \sum_{x \in A}X^x_{ab })$, additionally
 the final term can be seen as the difference of two expressions, both of which are the sums of $q_1 q_2$ random variables. Also, we know that $q_1 - q_2 \le 2\sqrt{n}$ and the expectation of a $0-1$ random variable is upper bounded by $1$.

Applying expectations term by term:

\begin{align*}
    \E[T_2] - \E[T_1] \ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + z q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \ge \frac{ \tau n\sqrt{n \log n}}{648}
\end{align*}
Using $s_{ij} - s_{kl} = \frac{T_2 - T_1}{|S_1| |S_2|}$, we get  $\E[s_{ij}] -\E [s_{kl}] = \frac{\E[T_2] - \E[T_1]}{|S_1||S_2|} \ge \frac{\tau \sqrt{\log n}}{648\sqrt{n}}$.
Both $s_{ij}$ and $s_{kl}$ have their respective numerator's variance to be $O(n)$ and thus overall variance bounded as $O(\frac{1}{n})$ (since the denominator of both terms is $\theta(n)$) implying the standard deviation of their difference is upper bounded by $O(\frac{1}{\sqrt{n}})$. Finally, $T_2 - T_1$ is also the sum of over $\frac{n}{12}$ independent random variables, thus we can use the Chernoff bound, for a large enough value of $\tau$, to conclude that $\E[T_2] - \E[T_1] > 0$ with probability at least $1 - \frac{1}{n^6}$.

{\bf Case 2:  $|B_2| > |B_1|$ i.e. $q_1 < q_2$ :}

\begin{align*}
    T_2 - T_1 &= z (\sum_{x \in A}(X^x_{cd } - X^x_{ab })) + (q_1 \sum_{x \in A}X^x_{cd } - q_2 \sum_{x \in A}X^x_{ab }) + z(\sum_{x \in B_2}X^x_{cd } - \sum_{y \in B_1}X^y_{ab }) + (q_1 \sum_{x \in B_2}X^x_{ab } - q_2 \sum_{y \in B_1}X^y_{ab }) \\
    &= z (\sum_{x \in A}(X^x_{cd } - X^x_{ab })) + q_2(\sum_{x \in A}(X^x_{cd } - X^x_{ab }) )  - (q_2 - q_1) \sum_{x \in A}X^x_{cd }
    + z(\sum_{x \in B_2}X^x_{cd } - \sum_{y \in B_1}X^y_{ab }) \\
    &  \quad + (q_1 \sum_{x \in B_2}X^x_{ab } - q_2 \sum_{y \in B_1}X^y_{ab })
\end{align*}

Since, $q_1, q_2 \le 4 \sqrt{n}$, we have $q_2 - q_1 \le 2\sqrt{n}$, additionally, the expectation of a $0-1$ random variable is upper bounded by $1$.

\begin{align*}
    \E[T_2] - \E[T_1] &\ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) z  + z q_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} %\\
    %&\ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) z  + z q_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}
\end{align*}

Working along the lines of the analysis in the previous case and using the fact that $(q_1 - q_2) z \le 2n\sqrt{n}$, we get 

\begin{align*}
    \E[T_2] - \E[T_1]   \ge \frac{\tau n\sqrt{n \log n}}{648} 
\end{align*}

Using a similar concentration argument as in the previous case, we can show that $\E[T_2] - \E[T_1] > 0$ with probability at least $\frac{1}{n^6}$.

\end{proof}
}



%Hide ends




\begin{proof}

Intuitively, this claim is true because the number of leaves that are used to generate the scores of both pairs $T_i, T_j$ and $T_k, T_l$ is sufficiently large  (at least $\frac{n}{16}$), and that these leaves all favor the pair $T_i, T_j$ (by at least $\theta\left( \sqrt{\frac{\log n}{n}} \right)$ each). Further, the number of leaves that are used to generate only one of the scores is bounded by $4 \sqrt{n}$. Consequently, these leaves do not alter the signal created by comparing the action of the leaves used to generate both scores. 

We introduce some notation to formalize the above intuition. Let $S_1 : = S \setminus (L_k \cup L_l)$ and $S_2 : = S \setminus (L_i \cup L_j)$. $S_1$ is the set of leaves used to compute the score $s_{kl}$ and $S_2$ is the set of leaves used to compute the score $s_{ij}$. Since $|L_k|, |L_l|, |L_i|, |L_j| \le 2 \sqrt{n}$, we can assume that $|S_1|, |S_2| \ge \frac{n}{16}$.  We can write $S_1 = A \cup B_1$ and $S_2 = A \cup B_2$ where $A := S_1 \cap S_2$, $B_1 : =  L_i \cup L_j$ and $B_2 := L_k \cup L_l$.



%Define $A := S_1 \cap S_2$, $B_1 := S_1 \setminus S_2$ and $B_2 := S_2 \setminus S_1$. Now $B_1 = L_i \cup L_j$ and $B_2 = L_k \cup L_l$. Thus $z := |A| \ge \frac{n}{16}$ and $q_1 := |B_1|, q_2 := |B_2| \le 4\sqrt{n}$. 
Using the condition on minimum edge length, it is not hard to see (Ref~Fig~\ref{fig:score_winner}) that :
\[ \forall x \in A: \E[X^x_{ij}]  - \E[X^x_{kl}] \ge \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \]
\[ \forall x \in B_2, y \in B_1: \E[X^x_{ij}]  - \E[X^y_{kl}] \ge \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \]

\esh{Should I include a proof of these two inequalities? Maybe rewrite them as a claim, so that we can push the proof to the appendix?}
\sk{May be not... since they seem pretty easy? Just state and say something like it is not hard to see... unless I am missing something.}
\esh{Done}

 Thus: 
\[s_{kl} = \frac{\sum_{x \in A}X^x_{kl} + \sum_{y \in B_1}X^y_{kl}}{|A| + |B_1|} \]

\[s_{ij} = \frac{\sum_{x \in A}X^x_{ij} + \sum_{x \in B_2}X^x_{ij}}{|A| + |B_2|} \]

% $s_{kl}$ and $s_{ij}$ are also random variables. 
We will compare the random variables $T_1 := |S_1||S_2| s_{kl}$ and $T_2 := |S_1||S_2| s_{ij}$. %If we can show that $T_2 - T_1 > 0$ with high probability, then we are done.
We know $q_1 := |B_1|, q_2 := |B_2| \le 4\sqrt{n}$. Let $z := |A|$.

\[ T_1 = z \sum_{x \in A}X^x_{kl} + q_2 \sum_{x \in A}X^x_{kl} + z \sum_{y \in B_1}X^y_{kl} + q_2 \sum_{y \in B_1}X^y_{kl} \]

\[ T_2 = z \sum_{x \in A}X^x_{ij} + q_1 \sum_{x \in A}X^x_{ij} + z \sum_{y \in B_2}X^y_{ij} + q_1 \sum_{y \in B_2}X^y_{ij} \]

\begin{flushleft}
{\bf Case 1: $|B_1| \ge |B_2|$ i.e. $q_1 \ge q_2$ :} 

Let $B'_1 \subset B_1$ be any subset such that $|B'_1| = |B_2|$. Then, we have:
\end{flushleft}
\begin{align*}
    T_2 - T_1 &= z (\sum_{x \in A}(X^x_{ij} - X^x_{kl})) + (q_1 \sum_{x \in A}X^x_{ij} - q_2 \sum_{x \in A}X^x_{kl}) + z(\sum_{x \in B_2}X^x_{ij} - \sum_{y \in B_1}X^y_{kl}) + (q_1 \sum_{x \in B_2}X^x_{kl} - q_2 \sum_{y \in B_1}X^y_{kl}) \\
    &\ge z (\sum_{x \in A}(X^x_{ij} - X^x_{kl})) + (q_1 \sum_{x \in A}X^x_{ij} - q_1 \sum_{x \in A}X^x_{kl}) + z(\sum_{x \in B_2}X^x_{ij} - \sum_{y \in B'_1}X^y_{kl}) - \sum_{y \in B_1 \setminus B'_1}X^y_{ij} \\
    & \quad + (q_1 \sum_{x \in B_2}X^x_{kl} - q_2 \sum_{y \in B_1}X^y_{kl})
\end{align*}

On the right hand side, %we can make the second term smaller by replacing it by $(q_2 \sum_{x \in A}X^x_{ij} - q_2 \sum_{x \in A}X^x_{kl})$, additionally
 the final term can be seen as the difference of two expressions, both of which are the sums of $q_1 q_2$ random variables. Also, we know that $q_1 - q_2 \le 2\sqrt{n}$ and the expectation of a $0-1$ random variable is upper bounded by $1$.

Applying expectations term by term:

\begin{align*}
    \E[T_2] - \E[T_1] \ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + z q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  \ge \frac{ \tau n\sqrt{n \log n}}{648}
\end{align*}
Using $s_{ij} - s_{kl} = \frac{T_2 - T_1}{|S_1| |S_2|}$, we get  $\E[s_{ij}] -\E [s_{kl}] = \frac{\E[T_2] - \E[T_1]}{|S_1||S_2|} \ge \frac{\tau \sqrt{\log n}}{648\sqrt{n}}$.
Both $s_{ij}$ and $s_{kl}$ have their respective numerator's variance to be $O(n)$ and thus overall variance bounded as $O(\frac{1}{n})$ (since the denominator of both terms is $\theta(n)$) implying the standard deviation of their difference is upper bounded by $O(\frac{1}{
\sqrt{n}})$. Finally, $T_2 - T_1$ is also the sum of over $\frac{n}{12}$ independent random variables, thus we can use the Chernoff bound, for a large enough value of $\tau$, to conclude that $\E[T_2] - \E[T_1] > 0$ with probability at least $1 - \frac{1}{n^6}$.


\begin{flushleft}
{\bf Case 2:  $|B_2| > |B_1|$ i.e. $q_1 < q_2$ :}
\end{flushleft}

\begin{align*}
    T_2 - T_1 &= z (\sum_{x \in A}(X^x_{ij} - X^x_{kl})) + (q_1 \sum_{x \in A}X^x_{ij} - q_2 \sum_{x \in A}X^x_{kl}) + z(\sum_{x \in B_2}X^x_{ij} - \sum_{y \in B_1}X^y_{kl}) + (q_1 \sum_{x \in B_2}X^x_{kl} - q_2 \sum_{y \in B_1}X^y_{kl}) \\
    &= z (\sum_{x \in A}(X^x_{ij} - X^x_{kl})) + q_2(\sum_{x \in A}(X^x_{ij} - X^x_{kl}) )  - (q_2 - q_1) \sum_{x \in A}X^x_{ij}
    + z(\sum_{x \in B_2}X^x_{ij} - \sum_{y \in B_1}X^y_{kl}) \\
    &  \quad + (q_1 \sum_{x \in B_2}X^x_{kl} - q_2 \sum_{y \in B_1}X^y_{kl})
\end{align*}

Since, $q_1, q_2 \le 4 \sqrt{n}$, we have $q_2 - q_1 \le 2\sqrt{n}$, additionally, the expectation of a $0-1$ random variable is upper bounded by $1$.

\begin{align*}
    \E[T_2] - \E[T_1] &\ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) z  + z q_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} %\\
    %&\ge z^2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}   + zq_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}} - (q_1 - q_2) z  + z q_1 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}  + q_1q_2 \frac{\tau \sqrt{\log n}}{9 \sqrt{n}}
\end{align*}

Working along the lines of the analysis in the previous case and using the fact that $(q_1 - q_2) z \le 2n\sqrt{n}$, we get 

\begin{align*}
    \E[T_2] - \E[T_1]   \ge \frac{\tau n\sqrt{n \log n}}{648} 
\end{align*}

Using a similar concentration argument as in the previous case, we can show that $\E[T_2] - \E[T_1] > 0$ with probability at least $\frac{1}{n^6}$.

\end{proof}



An immediate corollary of this claim, via an application of the union bound is that the highest scoring pair is in fact a sibling-tree pair. This gives an efficient algorithm that correctly combines subtrees of $T_S$ to form a larger subtree of $T_S$.


==> proofs/hellinger.tex <==
First, consider $H^2(Q^1_{a},Q^2_{a})$. These are both random variables corresponding to the query $(a,b,c)$, made on the two different trees. The support space of both random variables is $\{(a,b), (b,c) , (a,c) \}$. Let $p_1 := \Pr[Q^1(a,b,c) = (a,b)]$, $p_2 := \Pr[Q^1(a,b,c) = (b,c)]$ and $p_3 := \Pr[Q^1(a,b,c) = (a,c)]$. Similarly, let $q_1 := \Pr[Q^2(a,b,c) = (a,b)]$, $q_2 := \Pr[Q^2(a,b,c) = (b,c)]$ and $q_3 := \Pr[Q^2(a,b,c) = (a,c)]$. Let $d_1(a,b) = \alpha = d_2(a,c)$ and $d_1(a,c) = d_1(b,c) = d_2(a,b) =d_2(b,c) =\beta$. Observe that $\alpha \ge \frac{2}{3}$ since $d_1(a,p) = d_2(a,p) =\frac{1}{3}$. Also, $\beta - \alpha = \frac{2\rho}{\sqrt{n}}$. Using the definition of Hellinger distance : 

\[H^2(Q^1_{a},Q^2_{a}) = \frac{1}{2} ( (\sqrt{p_1} - \sqrt{q_1} )^2 + (\sqrt{p_2} - \sqrt{q_2} )^2 + (\sqrt{p_3} - \sqrt{q_3} )^2 )\].

We rewrite the probabilities in terms of the distances $\alpha$ and $\beta$:
\[
    p_1 = q_3 = \frac{2 \beta}{2(\alpha + 2 \beta)}
\]

\[
    p_2 = p_3 = q_1 = q_2 = \frac{\alpha + \beta}{2(\alpha + 2 \beta)}
\]


Next, we upper bound the quantity: $\sqrt{p_1} - \sqrt{q_1}$.

\begin{align*}
    \sqrt{p_1} - \sqrt{q_1} &=  \sqrt{\frac{2 \beta}{2(\alpha + 2 \beta)}} - \sqrt{\frac{\alpha + \beta}{2(\alpha + 2 \beta)}} \\
    &= \frac{\sqrt{2\beta} - \sqrt{\alpha+\beta}}{\sqrt{2(\alpha+2\beta)}} \\
    &\le \sqrt{\frac{4}{3}} (\sqrt{2\beta} - \sqrt{\alpha+\beta}) \qquad \text{( since $\alpha \ge \frac{2}{3}$)} \\
    &= \sqrt{\frac{4}{3}} \frac{\beta - \alpha}{(\sqrt{2\beta} + \sqrt{\alpha+\beta})} \qquad \text{( multiplying and dividing by $(\sqrt{2\beta} + \sqrt{\alpha+\beta})$)} \\
    &\le \frac{2\rho}{\sqrt{n}}  \qquad \text{( since $\alpha \ge \frac{2}{3}$)}
\end{align*}

We know $p_2 = q_2$. The final term of interest is $|\sqrt{p_3} - \sqrt{q_3}|$. Since $p_1 = q_3$ and $p_3 = q_1$, we get the upper bound - 
 $|\sqrt{p_3} - \sqrt{q_3}| \le \frac{2\rho}{\sqrt{n}}$.

Putting together these inequalities, we get 
$H^2(Q^1_{a},Q^2_{a}) \le \frac{1}{2} (\frac{8 \rho^2 }{n})$. Thus, for sufficiently small $\rho$, we get the desired result.

Now, consider $H^2(Q^1_{b,x},Q^2_{b,x})$. These are both random variables corresponding to the query $(a,b,x)$, made on the two different trees. The support space of both random variables is $\{(a,b), (b,x) , (a,x) \}$. Let $p_1 := \Pr[Q^1(a,b,x) = (a,b)]$, $p_2 := \Pr[Q^1(a,b,x) = (b,x)]$ and $p_3 := \Pr[Q^1(a,b,x) = (a,x)]$. Similarly, let $q_1 := \Pr[Q^2(a,b,x) = (a,b)]$, $q_2 := \Pr[Q^2(a,b,x) = (b,x)]$ and $q_3 := \Pr[Q^2(a,b,x) = (a,x)]$. Let $d_1(a,b) = \alpha$ and $ d_2(a,b) =\beta$. We have $d_1(a,x) = d_1(b,x) = d_2(a,x) = d_2(b,x) = 2$, since the associated unique path goes through the root for each of these pairs. %Observe that $\alpha \ge \frac{2}{3}$ since $d_1(a,p) = d_2(a,p) =\frac{1}{3}$. 
Again, we have  $\beta - \alpha = \frac{2\rho}{\sqrt{n}}$. Using the definition of Hellinger distance, we have : 

\[H^2(Q^1_{a},Q^2_{a}) = \frac{1}{2} ( (\sqrt{p_1} - \sqrt{q_1} )^2 + (\sqrt{p_2} - \sqrt{q_2} )^2 + (\sqrt{p_3} - \sqrt{q_3} )^2 )\].


\[
    p_1  = \frac{4}{2(4 + \alpha)} 
\]

\[q_1  = \frac{4}{2(4+\beta)} \]

\[
    p_2 = p_3  = \frac{2 + \alpha }{2(4 + \alpha)}
\]

\[
    q_2 = q_3  = \frac{2 + \beta }{2(4 + \beta)}
\]


Next, we upper bound the quantity: $\sqrt{p_1} - \sqrt{q_1}$.

\begin{align*}
    \sqrt{p_1} - \sqrt{q_1} &= \sqrt{2} \left( \frac{\sqrt{4+\beta} - \sqrt{4+\alpha}}{\sqrt{(4+\alpha)(4+\beta)}} \right) \\
    &\le \frac{1}{2 \sqrt{2}} (\sqrt{4+\beta} - \sqrt{4+\alpha}) \\
    &\le \frac{1}{2 \sqrt{2} (\sqrt{4+\beta} + \sqrt{4+\alpha})  } (\beta - \alpha) \\
    &\le \frac{1}{4 \sqrt{2}} \frac{ \rho}{\sqrt{n}}
\end{align*}

Now, consider $\sqrt{q_2} - \sqrt{p_2}$.

\begin{align*}
    \sqrt{q_2} - \sqrt{p_2} &= \frac{1}{\sqrt{2}} \frac{\sqrt{(2+\beta)(4+\alpha)}- \sqrt{(4+\beta)(2+\alpha)}}{\sqrt{(4+\alpha)(4+\beta)}} \\
    &\le \frac{1}{4 \sqrt{2}} (\sqrt{8 + \alpha \beta + 4 \beta + 2 \alpha} - \sqrt{8 + \alpha \beta + 2 \beta + 4 \alpha} ) \\
    &= \frac{1}{ 4\sqrt{2} (\sqrt{8 + \alpha \beta + 4 \beta + 2 \alpha} + \sqrt{8 + \alpha \beta + 2 \beta + 4 \alpha} ) } (2\beta - 2\alpha) \\
    &\le \frac{1}{8 \sqrt{2}} \frac{\rho}{\sqrt{n}}
\end{align*}

By an identical analysis, we have $\sqrt{q_3} - \sqrt{p_3} \le \frac{1}{8 \sqrt{2}} \frac{\rho}{\sqrt{n}}$. Putting together these inequalities, for $\rho \le \frac{1}{100}$, we get the desired result.


The same analysis as above gives $H^2(Q^1_{b,x},Q^2_{b,x}) \le \frac{10^-4}{4n}$. 


==> questions.tex <==
~\section{Questions}
\begin{enumerate}
    \item Is there a natural generalization of edge weight conditions under which we can recover the structure of the tree? - One hypothesis is the following condition - Let $N_v(\delta)$ represent the set of leaves within distance $\delta$ of leaf $v$. For all $\varepsilon, \delta > 0$, we have 
    \[|N_v((1+\varepsilon)\delta)| \le (1+10 \varepsilon)|N_v((1+ \varepsilon) \delta)| \]
    Roughly, this hypothesis says that the number of reachable leaves does not suddenly jump up as the distance from the 'source' leaf is increased by a small amount. Intuitively, this should be helpful because large jumps in the number of reachable leaves (corresponding to the $i+1$th cousins being added en masse to $N_v$) are accompanied by a significant increase in the distance and hence we get a sufficiently strong signal to distinguish between the $i$th and $(i+1)$th cousins. Observe that the above counterexample, with exponential weights, is ruled out by this condition.
    \item A necessary condition - consider siblings $a,b$ and their first cousin $c$ as the entire sub-tree rooted at the least common ancestor $e$ of $a,b,c$. To distinguish the first cousins from the siblings, we only get information from queries of the form $(a,b,x)$, $(a,c,x)$ and $(b,c,x)$. (there is no other information from which we can draw transitive closures - since $a,b,c$ are all indistinguishable to vertices outside the sub-tree rooted at $x$ since $d(e,a) =d(e,b) = d(e,c)$ from the ultrametric property).%(we get no information at all from queries of the form $(a,x,y)$ where $x,y$ are outside the sub-tree rooted at the least common ancestor of $a,b,c$)
    ~Let $d$ be the distance between the least common ancestor $f$ of $a,b$ and the leaf $c$. We need the distance $d$ to be at least $\frac{1}{n}$ of the total height of the tree, since we get at most $n$ signals from outside the sub-tree rooted at $e$.
\end{enumerate}

==> weights_old.tex <==

\section{Weight Reconstruction}
\label{sec:weight}
After reconstructing the topology of the tree, we turn our attention to the problem of reconstructing the weights on the edges. To do so, we will employ a stronger condition on the minimum weight of each edge - in particular, we assume that each edge has weight $\Omega(\frac{\log n}{\sqrt{n}})$. For estimating the weight of all but a constant fraction of the edges, the weaker condition we used to reconstruct tooplogy ( that each edge has weight $\Omega(\sqrt{\frac{\log n}{n}})$) will suffice. At the end of the process, we guarantee that the error on each edge is no more than a constant fraction (can be made arbitrarily small by changing the constant factor in the minimum weight condition). Recall that the tree is  normalized to have all root-leaf paths have length $1$. % \sk{Also mention that the tree is normalized to have all root-leaf paths have length 1.}

\ad{We should write the main theorem of this section at the beginning -- roughly here. There should then be some prose stating that }

We state the main result of this section below.

\begin{theorem}
\label{theorem:weights}
Let $T$ be a weighted full binary tree tree such that the weights induce an ultrametric on the distances between leaves and that the weight on each edge is at least $\tau  \frac{\log n}{\sqrt{n}}$, for some large constant $\tau$. Then, given access to the noisy query model (as described in Section~\ref{sec:model}) on the leaves of this tree, as well as the topology of the tree, we show that there exists an algorithm $\algweights$ that, with high probability, reconstructs the weight of each edge within an additive error $\kappa \frac{\log n}{\sqrt{n}}$, where $\tau \gg \kappa$).
\end{theorem}



%Instead of estimating the weight of each edge directly, we estimate the weight of the path from the root to every vertex v, denoted by $w_v$ in the tree within additive error of $\kappa \frac{\log n}{2\sqrt{n}}$. Using triangle inequality, the weight of each edge can be estimated within additive error $\kappa \frac{\log n}{\sqrt{n}}$ (we will assume that the minimum weight of an edge is $\tau \frac{\log n}{\sqrt{n}}$ where $\tau >> \kappa$).

Instead of estimating the weight of each edge directly, our algorithm estimates the weight of the path from the any leaf under a vertex $v$ to this vertex $v$, denoted by $h_v$ within additive error of $\kappa \frac{\log n}{2\sqrt{n}}$. Using triangle inequality, the weight of each edge can be estimated within additive error $\kappa \frac{\log n}{\sqrt{n}}$ %(we will assume that the minimum weight of an edge is $\tau \frac{\log n}{\sqrt{n}}$ where $\tau \gg \kappa$). 
We call this quantity $h_v$, as the height of vertex $v$.

Let $NL(v)$ represent the number of leaves in the sub-tree rooted at vertex $v$. We will follow a convention that for any leaf $v$ with right child $rc$ and left child $lc$, $NL(rc) \ge NL(lc)$. %\sk{Perhaps add here that the trees we consider can be assumed to be full wlog... i.e., no internal node has only one child, since in this case we can combine the edges below and above this node.} \esh{Now that we have combined the sections, this is already mentioned in the preliminaries}
We call a vertex $v$ heavy if $NL(v) \ge \alpha n +1$ where $\alpha = \frac{1}{6}$, otherwise, we call the vertex light. By definition, the root $r$ is a heavy vertex. By convention, for any leaf vertex $l$, $h_l = 0$. Let $P$ be the rightmost path from the root to a leaf (Fig~\ref{fig:rightmost}). Let the vertices on the path be in order - $r, v_1, v_2, ...,l^*$ where $l^*$ is the rightmost leaf in the tree. Let $f$ be the maximum index such that $v_f$ is a heavy vertex.

\begin{figure}
    \centering
     \includegraphics[width=8cm]{new_images/rightmost.png}
    \caption{Rightmost Path}
    \label{fig:rightmost}
\end{figure}

The algorithm $\algweights$ works in two phases. In the first phase, an estimate for the height of all vertices in the left subtree of every heavy vertex on the rightmost path is obtained, with additive error at most $\kappa \fs$ (and with high probability). Then, these estimates are in turn used to generate coarser estimates, with additive error upto $\kappa \frac{\log n}{\sqrt{n}}$ for the heights of the remaining vertices. An important tool, that we use to make these estimates, is Lemma~\ref{lemma:anchoring}, which implicitly connects the height of a heavy node and the height of some vertex in the subtree rooted at that heavy vertex.

{\bf Warm-Up : Estimating the heights of all Vertices in the Left Subtree of the Root}
Consider the root $r$, with left child $lc$ and right child $rc$. By our convention, we know that $rc$ is a heavy vertex. As an illustrative warm-up, we will first show how to estimate $h_v$ for any non leaf vertex $v$ in the sub-tree rooted at $lc$ (inclusive). Since $v$ is a non leaf vertex, it has at least one leaf vertex $a$ in its left sub-tree and at least one leaf vertex $b$ in its right sub-tree. Additionally, since $rc$ is a heavy vertex, we know there are at least $\alpha n$ leaves under it - indexed by $\{c_i\}_{i=1}^k$ where $k \ge \alpha n$ (Fig~\ref{fig:left_sub_root}). Let $X_i$ be the indicator random variable that query $Q(a,b,c_i)$ returns $(a,b)$ . Note that the $\{X_i\}$s are identical and independent random variables with expected value equal to $\frac{d(a,c_i) +d(b,c_i)}{2(d(a,b)+d(a,c_i) +d(b,c_i))} = \frac{4}{2(4+2h_v)} =\frac{1}{2+h_v}$.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{new_images/left_sub_root.png}
    \caption{Reconstructing the Left Subtree of the Root}
    \label{fig:left_sub_root}
\end{figure}

Based on the results of our queries, we generate $x_1, x_2, x_2..,x_k$ as realizations of the corresponding random variables, and compute $x=\frac{\sum_{i=1}^k x_k}{k}$.

\esh{Should I avoid the distinction between random variables and their realizations? Given that we have not got into this distinction in the topology reconstruction?}

\hide{
\begin{theorem}[Hoeffding Bound]
\label{theorem:hoeffding}
Let $y_1, y_2 ,.., y_k$ be $k$ iid random variables between $0$ and $1$, each with mean $y$, then: 
\[ |y- \frac{\sum_{i=1}^k y_k}{k}| \le \kappa_1 \sqrt{\frac{\log n}{k}} \] with probability at least $1 - \frac{1}{n^6}$.
where $\kappa_1$ is a sufficiently large constant ($\kappa_1 = 4$)
\end{theorem}
}
%moving Hoeffding to preliminaries


Using Theorem~\ref{theorem:hoeffding}
, we know that, with \ohp, $|x - \frac{1}{2+h_v}| \le \kappa_2 \fs$ where $\kappa_2 = \frac{\kappa_1}{\alpha}$.
Let $h'_v$ be a real number satisfying $x=\frac{1}{2+h'_v}$ (this can be found from $x$ by inverting the relation). Using the above result, we get $|h'_v-h_v| \le 12\kappa_2 \fs = \frac{12 \kappa_1}{\alpha} \fs$, since :
\begin{align*}
    |\frac{1}{2+h'_v} - \frac{1}{2+h_v}| &\le \kappa_2 \fs \\
    \implies |h_v -h'_v| &\le \kappa_2 (2+h_v)(2+h'_v) \fs\\
    &\le 12 \kappa_2 \fs
\end{align*}

Note that, with high probability:  $\frac{1}{6} \le \frac{1}{2+h'_v} \le 1$ (using the Chernoff bound again) implies that$ -1 \le h'_v \le 2$, and we already know that $\frac{1}{3} \le \frac{1}{2+w_v} \le \frac{1}{2}$.

{\bf Estimating the heights of Heavy Vertices on the Rightmost Path}
Next, we show that it is possible to estimate $h_{v_l}$ for any vertex $v_l$ on the path $P$ with $1\le l \le f$. Consider vertex $v_l$, since $l \le f$, we know that $NL(v_l) \ge \alpha n +1$. Thus, we know that there are at least $k \ge \alpha n$ pairs  of leaves $(a_i,b_i)$ such that $a_i$ is in the left sub-tree of $v_l$ and $b_i$ is in the right sub-tree of $v_l$. We know that there is at least one leaf $c$ in the left subtree of the root $r$. Again, let $X_i$ be the indicator variable that the query on triple $(a_i,b_i,c)$ returns $(a_i,b_i)$. We see that they are iid random variables, each with mean $\frac{1}{2+h_{v_l}}$. Let $x=\frac{\sum_{i=1}^k x_k}{k} $, where the $\{x_i\}$s are realized values of the corresponding random variables. Using Theorem~\ref{theorem:hoeffding}, as before, we have with \ohp, an estimate $h'_{v_l}$ such that $|h'_{v_l}-h_{v_l}| \le  \frac{12 \kappa_1}{\alpha} \fs$. %\esh{Having some trouble proving that $\E[w'_l] = w_l$ due to the inverse relationship...will see if it is really needed}

\sk{Here are somewhere around here would be a good place to make the point, that if we ever encounter a node with two heavy children, based on what we have said, the whole problem is solved...}

Additionally, if there is a single vertex on the path with two heavy children,  we can recover the weight (upto constant additive error) of every edge. This is because we can use the leaves on the opposite side to estimate the root to vertex distance for any vertex in a subtree (using a method similar to the one used to estimate $h_v$ for any $v$ in the left subtree of the root).

Finally, we note that the same method can be used to estimate $h_{v_{f+1}}$ with a constant blowup in additive error, since $NL(v_{f+1}) \ge \frac{\alpha n}{2}$. \sk{With a little care we can estimate this height without any blowup in additive error.}

\subsection{Anchoring Leaves to a Vertex on Path $P$}

We show an important result that implictly connects the height of a heavy vertex with the height of vertex in its subtree.

\begin{lemma}
\label{lemma:anchoring}
Let $v$ be an internal vertex of the tree and let $v_l$ be a heavy vertex on path $P$ such that $v_l$ is an ancestor of vertex $v$, and has $k$ leaves in the sub-tree not containing $v$, where $k \ge 100.$% is at least a reasonably large constant. 
Then, the probability $p$ that the query $Q(a,b,c)$ gives $(a,b)$ can be estimated to within an additive error of $ \kappa_1 \sqrt{\frac{log k}{k}}$, where $a$ and $b$ are leaves in distinct subtrees of $v$ and $c$ is a  vertex in the subtree of $v_l$ not containing $v$. Additionally, if $p'$ is the estimate, then $\mathbb{E}[p'] = p$. We say that vertex $v$ has been anchored to vertex $v_l$ to obtain this estimate.
\end{lemma}

\begin{proof}

%To begin, note that we already have an estimate $w'_{v_l}$ for $w_{v_l}$ such that $|w'_{v_l} - w_{v_l}| \le \kappa_3 \fs$ and $\mathbb{E}[w'_{v_l}] = w_{v_l}$.
Since $v$ is an internal vertex, there exists two leaves $a$ and $b$ such that they are in opposite subtrees of $v$. Index the leaves in the sub-tree of $v_l$ not containing $v$ as $c_1,c_2,..c_k$. 

Let $c$ be any vertex in $c_1,c_2,...c_k$. Let $p$ be the probability that $Q(a,b,c)$ gives the answer $(a,b)$. (This probability is the same for all $c_i$.)

Since $d(a,b) = 2h_v$ and $d(a,c) = d(b,c) = 2h_{v_l}$, $p = \frac{h_{v_l}}{2h_{v_l} + h_v}$. Let $X_i$ be the indicator variable that the query on triple $(a,b,c_i)$ returns $(a,b)$. The $X_i$'s are iid random variables, each with mean $\frac{h_{v_l}}{2h_{v_l} + h_v}$. Let $x=\frac{\sum_{i=1}^k x_i}{k} $, where the $\{x_i\}$s are realized values of the corresponding random variables. Using the Hoeffding bound (Theorem~\ref{theorem:hoeffding}), we know that $|p -x| \le \kappa_1 \sqrt{\frac{\log k}{k}}$. Thus, we get an estimate $x$ with the desired approximation. Further, using the linearity of expectation, $\E[x] = p$.

%Let $u_v := \frac{d(a,c) -d(a,b)}{d(a,c)}$. Note that $d(a,b) = 2h_v$ and $d(a,c) = d(b,c) = 2h_{v_l}$.  %\\\Thus, $u_v = \frac{w_v - w_{v_l}}{1-w_{v_l}}$ $w_v = w_{v_l} + u_v. (1-w_{v_l})$. Since $v_l$ is a heavy vertex, we already have estimate $w'_{v_l}$ with additive error at most $\kappa_3 \fs$. Let $\varepsilon_1$ represent this additive error. Assume that we have an estimate $u'_v$ for $u_v$ with additive error $\varepsilon_2 = \kappa_5 \sqrt{\frac{\log k}{k}}$ and $\E[\varepsilon_2] =0$. Note that $\varepsilon_1 \le  \varepsilon_2$ if $k \le n$. We claim that this assumption suffices to obtain the desired result. Let $w'_v = w'_{v_l} + (1-w'_{v_l}) u'_v $. Observe that we can write $w'_{v_l} = w_{v_l} + \varepsilon_1$ and $u'_v = u_v + \varepsilon_2$. Thus, $w'_v = w_{v_l} + u_v (1-w_{v_l}) + \varepsilon_1(1-u_v + \varepsilon_2) + \varepsilon_2(1-w_{v_l})$. Note that $u_v, w_{v_l} \in (0,1)$ implies that the absolute value of the error term is at most $|\varepsilon_1|(1+|\varepsilon_2|) + |\varepsilon_2| \le 1.1 |\varepsilon_1|+ |\varepsilon_2| $ (by assuming that $\varepsilon_2  < 0.1$ , which is true for all reasonable large constant values of $k$). 
%\esh{Add proof for expected value}
%We know that $\mathbb{E}[\varepsilon_1] = \mathbb{E}[\varepsilon_2] =0$, and that they are independent random variables (since the sets of queries used to estimate them are mutually disjoint), thus $\mathbb{E}[\varepsilon_1 \varepsilon_2] = 0$. Applying linearity of expectation gives $\mathbb{E}[w'_{v_l}] = w_{v_l}$.

%[[[Note: Some issues with constants here!!]]]

%Now, to generate the estimate $u'_v$, observe that each random variable $X_i$ has mean $\frac{d(a,c_i) +d(b,c_i)}{2(d(a,b)+d(a,c_i) +d(b,c_i))}$. Dividing numerator and denominator by $d(a,c_i)$, the mean is equal to $\frac{1}{3-u_v}$. We can again use Lemma~\ref{lemma:hoeffding} as before to get an estimate $u'_v$ with the desired property with \ohp.

\end{proof}

This lemma gives us an estimate for the height of any internal vertex $v$ in the left sub-tree of any heavy vertex $v_l$ on path $P$,i.e, $1 \le l \le f$. We know that $v_l$ is trivially an ancestor of $v$ and has at least $\frac{\alpha n}{2}$ leaves in the opposite sub-tree. Thus, using Lemma~\ref{lemma:anchoring}, we get an estimate $p'$ for $ p = \frac{h_{v_l}}{2h_{v_l} + h_v}$ with additive error no greater than $\frac{2\kappa_1}{\alpha} \fs$. We can rewrite the relation between $p, h_v$ and $h_{v_l}$ as 
\[ h_v = \frac{h_{v_l} (1-2p)}{p} \] Consider the bivariate function $f(a,b) = \frac{a(1-2b)}{b}$. We have $ \frac{\partial f }{\partial a} = \frac{1}{b} - 2$. Similarly, $ \frac{\partial f }{\partial b} = -\frac{a}{b^2} $. The ``true'' values $h_{v_l}$ and $p$ satisfy $h_{v_l} \in [0,1]$ and $p \in [1/3,1/2]$. Since we have subconstant additive error in the estimates for both quantities, we can restrict the range of interest for the variables $a$ and $b$ as $a \in [0,5/4]$ and $b \in [1/4, 2/3]$.   Thus, we have $|\frac{\partial f }{\partial a}| \le 5/4$ and $| \frac{\partial f }{\partial b}| \le \frac{5/4}{(1/4)^2} = 20$. \sk{Did you mean to bound the partial with respect to $b$ here? If so, the bound on magnitude is 9, not 1/4.} We need to find $f(h_{v_l},p)$ but only have estimates $h'_{v_l}$ and $p'$. Using the above two bounds on the partial derivatives, we conclude that $|f(h_{v_l},p) - f(h'_{v_l},p')| \le  \frac{45\kappa_1}{\alpha} \sqrt{\frac{\log n}{n}}$. Thus, $f(h'_{v_l},p')$ gives a good estimate for $p$.


This completes the description of the first phase of the algorithm $\algweights$, which estimates the weights of all descendants of heavy vertices (inclusive).
%\sk{Is the last expression slightly changed by the correction above? Also, could we avoid a proliferation of $\kappa 's$ and use the same $\kappa$ throughout with appropriate constants if that is possible?} \esh{Have fixed these issues}



\subsection{Internal Vertices in the Sub-tree of $v_{f+1}$}

For all vertices except those in the sub-tree of $v_{f+1}$ we have shown that we can estimate their heights to within additive error $O(\fs)$. For  the vertices under $v_{f+1}$, we have a slightly worse bound of $O(\frac{\log n}{\sqrt{n}})$ on the additive error in their height estimates.

We now focus on any internal vertex $v$ in the sub-tree of $v_{f+1}$ (not inclusive). We know there are at least 
$(1-\alpha) n -1$ leaves in the left sub-trees of all vertices $\{v_l\}$ for $l =0$ to $l=f$ (where $v_0 = r$, the root of the tree). Since we have started with $\alpha < 0.49$, there are at least $\frac{n}{2}$ such leaves, distributed among the left sub-trees of $\{v_l\}$ for $l =0$ to $f$. Consider only the vertices $v_l$ in this set such that the left sub-tree (of that vertex) have at least $\frac{n}{4(f+1)}$ leaves. Since there are at most $f$ vertices left out, the leaves covered by this selected set is at least $\frac{n}{2} - f.\frac{n}{4(f+1)} \ge \frac{n}{4}$. Let the selected vertices be re-indexed as $t_1, t_2, ...t_k$. Let $j_i$ be the number of leaves in the left sub-tree of $t_i$. Consider the query $Q(a,b,c)$ where $a$ and $b$ are leaves in distinct subtrees of $v$ and $c$ is a leaf in the subtree of $t_i$. Let $p_i$ be the probability that the answer of this query is $(a,b)$. Note that $p_i = \frac{h_{t_i}}{2h_{t_i} + h_v}$.  Using Lemma~\ref{lemma:anchoring} and using $t_i$ as an anchor of $v$, we get an estimate $x_i$ for $p_i$ . We know that, with high probability, $|x_i - p_i| \le \kappa_1 \sqrt{\frac{log j_i}{j_i}}$ - we will henceforth condition upon this event (and use the union bound to argue that all such events happen with high probability). Also, Lemma~\ref{lemma:anchoring} tells us that $\E[x_i] = p_i$. Additionally, we know that $\sum_{i=1}^k j_i \ge \frac{n}{4}$. 


\hide{
\begin{definition}[Bounded Difference Property]
\label{def:bounded}
We say that $g: \mathbb{D}^n \rightarrow \mathbb{R}$ for some domain $\mathbb{D} \subseteq \mathbb{R}$ satisfies the bounded difference property with constants $L_1, L_2 \cdots L_n$ if for all $i \in [n]$ and $x_1,x_2,\cdots x_n, x'_i \in \mathbb{D}$, we have the property that :
\[ |g(x_1,x_2,x_3 \cdots x_n) - g(x_1,x_2, \cdots x_{i-1},x'_i,x_{i+1}, \cdots x_n)| \le L_i \]
 
\end{definition}
}

Define $g(x_1,x_2,..x_k) := \frac{\sum_{i=1}^k j_i x_i }{\sum_{i=1}^k j_i}$  on the product of intervals $I_1 \times I_2 \cdots I_n$ where each $I_i$ is an interval of size $2 \kappa_1 \sqrt{\frac{log j_i}{j_i}}$ around $p_i$. We know that $g$ satisfies the bounded difference property (Definition~\ref{def:bounded}) with respect to $x_i$ with difference $L_i = \frac{8 j_i \kappa_1 \sqrt{\log n}}{\sqrt{j_i} n} = \frac{8  \kappa_1 \sqrt{ j_i \log n}}{n}$.

\hide{
\begin{theorem}[McDiarmid's Inequality]
\label{theorem:McDiarmid}
Suppose $X_1, X_2,...X_n$ are independent random variables and function $g : \mathbb{D}^n \rightarrow \mathbb{R}$  for some domain $\mathbb{D} \subseteq \mathbb{R}$ satisfies the bounded differences property with constants $L_1, L_2, ...L_k$, then:

\[\Pr[|g(X_1,X_2,..X_k) - \mathbb{E}[g(X_1,X_2,..X_k)]| \ge t] \le 2\exp(-\frac{2t^2}{\sum_{i=1}^k L^2_i})\]

\end{theorem}
}

We appeal to McDiarmids's inequality (Theorem~\ref{theorem:McDiarmid}). Using linearity of expectation, we know that $\mathbb{E}[g(X_1,X_2,..X_k)] =   \frac{ \sum_i \frac{j_i h_{t_i}}{(2h_{t_i} + h_v)}}{ \sum_i j_i}$.%\esh{This might need an expanded proof, since it uses properties of previous estimates}
Set $t = \frac{ 24 \kappa_1 \log n}{\sqrt{n}}$. We know that $\sum_{i=1}^k L^2_i = \sum_{i=1}^k \frac{64 \kappa_1^2 j_i \log n}{n^2}$.
 Since $ n \ge \sum_{i=1}^k j_i \ge \frac{n}{4} $, we have 
 \[ \frac{64 \kappa^2_1 \log n}{n} \ge \sum_{i=1}^k L^2_i \ge \frac{16 \kappa^2_1 \log n}{n}\].
 
 Thus, with probability at most $\frac{1}{n^6}$, we have $|g(x_1,x_2,..,x_k) -  \frac{ \sum_i \frac{j_i h_{t_i}}{(2h_{t_i} + h_v)}}{ \sum_i j_i}| \ge \frac{ 24 \kappa_1 \log n}{\sqrt{n}}$. %Our final estimate is thus set to $w'_v = g(x_1,x_2,..,x_k)$.
 
 Let $K' = g(x_1,x_2 \cdots x_n)$. To finish the proof, we show how to recover $h_v$ from $K'$. We define a multivariate function $F$ that operates on inputs $a \in \mathbb{R}$ and $b = (b_1, b_2 ,\cdots b_k) \in \mathbb{R}^k$. 
 
 \[ F(a,b) :=\frac{ \sum_{i=1}^k \frac{j_ib_i}{2b_i + a}}{\sum_i j_i} \]
 
 \sk{Again slight mismatch of notation --- $b_i$ should be replaced by $V_i$?} \esh{I went with $a$ and $b$ as generic placeholder variables rather than have names that correspond to specific values}
 
 Alternatively, we write $F(a,b) = \frac{\sum_{i=1}^k j_i f(a,b_i) }{\sum_i j_i}$ where $f(a,b_i) = \frac{b_i}{2b_i + a}$, i.e., we write $f$ as a convex combination of $k$ functions. For ease of notation, we call $\alpha_i = \frac{j_i}{\sum_{a=1}^k j_a}$. Note that all $\alpha > 0$ and $\sum_i \alpha_i = 1$.

 
  Let $H = \{ h_{t_1}, h_{t_2}, \cdots h_{t_k}\}$ and $H' = \{ h'_{t_1}, h'_{t_2}, \cdots h'_{t_k}\}$.
  
   
 
 
 Intuitively, we want to invert the value $K'$ of the function $f$ using our estimates $H'$ to obtain an estimate $h'_v$ that is close to $h_v$. To do so, we first prove some properties of each function $f(a,b_i)$.
 
 \[ \frac{\partial f(a,b_i)}{\partial b_i} = \frac{a}{(2b_i+a)^2} \]
 
  \[ \frac{\partial f(a,b_i)}{\partial a} = \frac{-b_i}{(2a_i+b)^2} \]
  
  %Note that in our domain of interest, 
  We know that $h_{t_i} > h_v$ for all indices $i$. Additionally, $h_{t_i} \ge \tau \frac{\log n}{\sqrt{n}}$ where $\tau$ is a large constant. \sk{One more notational issue --- $v_i$, or the subset of heavy vertices you selected, which you named $t_i$? I think the latter, but this proof is  complicated and confusing and the notation has to be simple and elegant ... and correct.}\esh{Fixed by changing to $t_i$ throughout}
 
 First, we show how the algorithm come up with an estimate $h'_v$ for the height of vertex $v$. This claim completes the description of the algorithm $\algweights$.
 
 \begin{claim}
 There exists a unique real number $h'_v$ such that $F(h'_v,H') = K'$. Additionally, this real number can be found using numerical methods given $K$ and $H'$.
 \end{claim}
 
\begin{proof}
 Fix the second argument of $F$ to be $H'$, $F$ is now a univariate function on the first argument. This function is monotone decreasing since each univariate function $f(a,h_{v_i})$ is monotone decreasing and $F(a,H')$ is a convex combination of these functions. Thus, $F$ is invertible. Further, simple numerical methods such as binary search can be used to find $h'_v$ such that $F(h'_v,H') = K'$.  
\end{proof}



Let $K = F(h_v,H)$. Recall that $K' =F(h'_v,H') $ and with high probability, $|K - K'| \le \frac{24 \kappa \log n}{\sqrt{n}} $.
 
 
Now, we show a simplified analysis, for the case that $h'_v \le h'_{t_i}$ for $i \in [k]$ (i.e, the estimate $h'_v$ satisfies some natural conditions that arise from the relative position of the vertex $v$ and the vertices $v_1, v_2 \cdots v_k$ in the tree). We will later show a more involved analysis for when our estimate does not satisfy these conditions.

For sake of contradiction, assume that $|h'_v - h_v| \ge \Delta \frac{\log n}{\sqrt{n}}$, where $\Delta = 
\frac{\tau}{10}$. Since  $|K - K'| \le \frac{24 \kappa \log n}{\sqrt{n}} $, we get:

\begin{align*}
    |\sum_i \alpha_i \{f(h_v,h_{t_i}) - f(h'_v,h'_{t_i}) \}| &\le \frac{24 \kappa \log n}{\sqrt{n}} \\
     \implies |\sum_i \alpha_i \{(f(h_v,h_{t_i}) - f(h'_v,h_{t_i})) + (f(h'_v,h_{t_i}) - f(h'_v,h'_{t_i})) \}|  &\le \frac{24 \kappa \log n}{\sqrt{n}}     \tag{*}
\end{align*}
 
We now bound each term in the above expression, for each $i \in [k]$. Using the intermediate value theorem on the (continuous) univariate function $f(a,h_{t_i})$ (Second argument fixed to be $h_{t_i}$) in the interval $[h_v,h'_v]$, we know there exists $x \in [h_v,h'_v]$ such that:

\begin{align*}
    A := |f(h_v,h_{t_i}) - f(h'_v,h_{t_i})| &=  \left | \frac{\partial f(a,h_{t_i})}{\partial a} \right|_{a=x}. |h_v -h'_v| \\
    &= \left | \frac{h_{t_i}}{(2h_{t_i} + x)^2} \right|. |h_v -h'_v|
\end{align*}


 Using the intermediate value theorem on the univariate function $f(h'_v,b)$ (first argument fixed to be $h'_{v}$) in the interval $[h_{t_i},h'_{t_i}]$, we know there exists $y \in [h_{t_i},h'_{t_i}]$ such that:

\begin{align*}
    B := |f(h'_v,h_{t_i}) - f(h'_v,h'_{t_i})| &=  \left | \frac{\partial f(h'_v,b)}{\partial b} \right|_{b=y}. |h_{t_i}-h'_{t_i}| \\
    &= \left | \frac{h'_v}{(2y + h'_v)^2} \right|. |h_{t_i} -h'_{t_i}|
\end{align*}

Since $|h'_{t_i} - h_{t_i} | \le 12 \kappa_2 \fs$ and $h_{t_i} \ge \tau \frac{\log n}{\sqrt{n}}$, we know that $2h'_{t_i} \ge h_{t_i} \ge h'_{t_i}/2 $. We also know that $h'_v \le h'_{t_i}$ by our assumption and hence $h'_v \le 2h_{t_i}$ which would imply that $x \le 2h_{t_i}$. Thus, we have $\frac{h_{t_i}}{(2h_{t_i}+x)^2} \ge \frac{h_{t_i}}{9h^2_{t_i}} = \frac{1}{3h_{t_i}}$ and $\frac{h'_v}{(2y + h'_v)^2} \le \frac{1}{2h'_{t_i}}$. Note that using the triangle inequality $|A| - |B| \ge ||A| - |B||$. Thus, as long as $\tau$ is large enough ($\tau > 480 \kappa_4, 480 \kappa_2$), we know that $|A| - |B| \ge \tau/20 \frac{\log n}{\sqrt{n}}$. Substituting this into inequality~*, we get a contradiction, leading us to conclude that $|h'_v - h_v| \le \Delta \frac{\log n}{\sqrt{n}}$ (with high probability).



{\bf Moving Past the Height Estimate Assumption : } Now, let us consider the case that there exists some $i$ such that $h'_v > h_{t_i} $. In this event, we will instead use the smallest such height $U = \min_i \{h'_{t_i}\}$ as an estimate for $h'_v$. We show that $|U - h_v| \le \Delta \frac{\log n}{\sqrt{n}}$ with high probability. Assume that  $|U - h_v| > \Delta \frac{\log n}{\sqrt{n}}$, for sake of contradiction. We will show similar bounds on the expressions $A$ and $B$ from the above proof. First, we lower bound $|A|$. Consider the (continuous) univariate function $f(a,h_{t_i})$ on the intervals $[h_v,U]$ and $[U,h'_v]$. Using the intermediate value theorem on both intervals, there exists $x_1 \in [h_v,U] $ and $x_2 \in [U,h'_v]$ such that:

\begin{align*}
    A := |f(h_v,h_{t_i}) - f(h'_v,h_{t_i})| &=  \left ( \frac{\partial f(a,h_{t_i})}{\partial a} \right)_{a=x_1}. |U -h_v| +  \left ( \frac{\partial f(a,h_{t_i})}{\partial a} \right)_{a=x_2}. |h'_v -U|\\
    &\ge \left ( \frac{\partial f(a,h_{t_i})}{\partial a} \right)_{a=x_1}. |U -h_v| \\
    &= \left | \frac{h_{t_i}}{(2h_{t_i} + x_1)^2} \right|. |U -h_v|
\end{align*}

Thus, with similar reasoning as before, we have $\frac{h_{t_i}}{(2h_{t_i}+x_1)^2} \ge \frac{h_{t_i}}{9h^2_{t_i}} = \frac{1}{3h_{t_i}}$ since $x_1 \le h'_{t_i}$ for all $i$.

Now, to upper bound $B$, we consider the (continuous) univariate function $f(h'_v,b)$ on the interval $[h_{t_i},h'_{t_i}]$, we know there exists $y \in [h_{t_i},h'_{t_i}]$ such that:

\begin{align*}
    B := |f(h'_v,h_{t_i}) - f(h'_v,h'_{t_i})| &=  \left | \frac{\partial f(h'_v,b)}{\partial b} \right|_{b=y}. |h_{t_i}-h'_{t_i}| \\
    &= \left | \frac{h'_v}{(2y + h'_v)^2} \right|. |h_{t_i} -h'_{t_i}|
\end{align*}

Consider the univariate function $g(x) = \frac{x}{(2c+x)^2}$. Note that $g(x) > 0$ if $c,x > 0$. Thus, $|g(x)|$ (for $c,x > 0$) is maximized at the same point as $g(x)$ which is at $x = 2c$. Thus, $\frac{h'_v}{(2y + h'_v)^2} \le \frac{2y}{16y^2} = \frac{1}{8y} \le \frac{1}{4h_{t_i}}$. Similar analysis as before leads us to a contradiction ( we can show that $|A| \ge 2|B|$, which suffices to prove the result).






